Robust Training in High Dimensions via Block Coordinate Geometric Median Descent

Geometric median (\textsc{Gm}) is a classical method in statistics for achieving a robust estimation of the uncorrupted data; under gross corruption, it achieves the optimal breakdown point of 0.5. However, its computational complexity makes it infeasible for robustifying stochastic gradient descent (SGD) for high-dimensional optimization problems. In this paper, we show that by applying \textsc{Gm} to only a judiciously chosen block of coordinates at a time and using a memory mechanism, one can retain the breakdown point of 0.5 for smooth non-convex problems, with non-asymptotic convergence rates comparable to the SGD with \textsc{Gm}.

==> bgmd_algo_block.tex <==
\begin{algorithm}[t]
        \SetAlgoLined
        \textbf{Initialize:}
        estimate: $\vx_0 \in \sR^d$, step-size: $\gamma$, 
        memory: $\mM_0 = \textbf{0} \in \sR^{b \times d}$,  Block Coordinate Selection operator: $\gC_k(\cdot)$, Geometric Median operator: \textsc{Gm}($\cdot$) \\
        %Given samples $\gD = (\vx_t, \vy_t)_{t=0}^{\infty}$\\
        \For{epochs \; t = 0, \dots , until convergence}
        {
            Select set $\gD_t=\{i_1, \dots, i_b\}$ \\
            Obtain : $\vg_t^{(i)} := \nabla f_i(\vx_t) , \; \forall i \in \gD_t$\\
             Let $\mG_t \in \sR^{b \times d}$ s.t. each row $\mG_t[i, :] = \vg_t^{(i)}$
             $\mG_t = \gamma \mG_t + \mM_t$ \quad (Memory Augmentation)\\
             $\boldsymbol{\Delta}_t := \mathcal{C}_k (\mG_t)$ \quad (Select top $k$ columns via Algo \ref{algorithm:co_sparse_approx})\\
             $\mM_{t+1} = \mG_t - \boldsymbol{\Delta}_t $ \quad (Update memory)\\
             $\Tilde{\vg}_t := \textsc{Gm}(\boldsymbol{\Delta}_t)$ \quad(Robust Aggregation in $\sR^k$)\\
             $\vx_{t+1}:= \vx_t - \Tilde{\vg}_t$ \quad (Global model update)\\
        }
        %\caption{Robust BCD with Memory (BCDm) \textbf{(This work)}} %\textsc{Gm}}
        \caption{Block \textsc{Gm} Descent (\textsc{BGmD})}
        \label{algorithm:full}
\end{algorithm}%\DecMargin{1 em}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]

    \SetAlgoLined
    \textbf{Input:} \; $\mG_t \in \sR^{n \times d},\; k $ \\
    \For{coordinates \; j = 0, \dots , d-1}
    {
        $s_j \gets \|\mG_t[:, j]\|^2$ \; (norm along each dimension)
    }
    Sample set $\sI_k$ of $k$ dimensions with probabilities proportional to $s_j$\\
    $\gC_k(\mG)_{i, j\in \sI_k} =  \mG_{i, j} , \; 
        \gC_k(\mG)_{i, j\notin \sI_k} = 0 $ \\
    \textbf{Return:} $\gC_k(\mG)$
    \caption{Block Coordinate Selection Strategy}
    \label{algorithm:co_sparse_approx}
\end{algorithm}%\DecMargin{1em}


==> experiment.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In this section, we describe our experimental setup and present our empirical findings. 
\textbf{Experimental Setup.}
% \subsection{Corruption Simulations}
We use two important optimization setups for our experiments: 

\textbf{(a) Homogeneous}: We trained a moderately large LeNet \cite{lecun1998gradient} style CNN with 1.16M parameters on the challenging Fashion-MNIST \cite{xiao2017fashion} dataset in the \textit{vanilla mini batch} setting with 32 parallel mini-batches each with batch size 64. The training data was \textbf{i.i.d} among all the batches at each epoch. We use initial learning rate of 0.01 which was decayed by $1\%$ at each epoch. Each experiment under this setting was run for \textbf{50 epochs} (full passes over training data). % In (Figure \ref{figure:fmnist.lenet}) we plot the convergence and accuracy under different levels of \textit{Additive Corruption}. For this setting, \textsc{BGmD} was run with block size $k = 0.05 \times d$ where $d$ is total number of parameters in LeNet.   

\textbf{(b) Heterogeneous}: Our theoretical results (Theorem ~\ref{theorem:nonconvex-simple},~\ref{theorem:plc-simple}) are established without any assumption on how the data is distributed across batches. We verify this by training an 18-layer wide ResNet \cite{he2016deep} with 11.2M parameters on CIFAR 10 \cite{krizhevsky2012imagenet} in a \textbf{federated learning} setting \cite{mcmahan2017communication}. In this setting, at each iteration 10 parallel clients compute gradients over batch sizes of 128 and communicate with the central server. The training data was distributed among the clients in a \textbf{non i.i.d} manner only once at the beginning of training\footnote{The non-i.i.d data distribution strategy is described in supplementary.}.   
Each experiment was run for \textbf{200 epochs} with an initial learning rate 0.1 and warm restarted via cosine annealing decay.

For both the experiments we used the categorical cross entropy loss plus an $\ell_2$
%%%%%%%%%%%%%%%%%%%%
\setlength{\intextsep}{0pt}%
\setlength{\columnsep}{6pt}%
\begin{wrapfigure}{r}{0.45\textwidth}
\centering
\subfloat{\includegraphics[width=0.22\textwidth]{figs/neurips/attack/im_sample.png}}
\subfloat{\includegraphics[width=0.22\textwidth]{figs/neurips/attack/im_sample_sp.png}}
\caption{\label{figure:time_complexity} \footnotesize{\textbf{Example of Feature Corruption:} (left) 
clean sample (right) corruption via impulse noise}}
\end{wrapfigure}
%%%%%%%%%%%%%%%%%%%%
regularizer with weight decay value of $1\mathrm{e}{-4}$. All the experiments are performed on a single 12 \textsc{GB Titan Xp} GPU. For reproducibility, all the experiments are run with deterministic \textsc{CuDNN} back-end. Further, each experiment is repeated 5 times with different random seeds and confidence interval is noted. Table~\ref{table:fmnist_table} and Table~\ref{table:cifar_table} provide a summary of the results \footnote{\label{appx.tables} Due to space constraint we are only able to put a small subset of our experiments. Please check the supplementary section for a more complete set of results.} %All results reported also report the confidence interval across runs. 
\input{arxiv/result_table_main}

\begin{figure}[t]
\subfloat[\footnotesize{No corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/fmnist/clean.png}}
\subfloat[\footnotesize{10\% Corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/fmnist/f.ip.10.png}}
\subfloat[\footnotesize{20\% Corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/fmnist/f.ip.20.png}}
\subfloat[\footnotesize{40\% Corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/fmnist/f.ip.40.png}} 
\caption{\footnotesize{\textbf{Robustness to Feature Corruption}: We compare  test set performance of different schemes as a function of \textbf{wall clock time} for training Fashion MNIST in i.i.d setting. These experiments are performed in presence of increasing the fraction samples corrupted with \textbf{impulse noise}. At 40\% corruption \textsc{SGD} diverged and thus does not appear in the plot. Observe that \textsc{BGmD} is able to maintain high accuracy in even presence of strong corruption and is at least \textsc{GmD} while attaining at least 3x speedup over \textsc{GmD}.}}
\label{figure:fmnist.image_corr}
\end{figure}
\begin{figure}[t]
\subfloat[\footnotesize{No corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/fmnist/clean.png}}
\subfloat[\footnotesize{10\% Corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/fmnist/bf.10.png}}
\subfloat[\footnotesize{20\% Corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/fmnist/bf.20.png}}
\subfloat[\footnotesize{40\% Corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/fmnist/bf.40.png}}  
\caption{\footnotesize{\textbf{Robustness to Gradient Corruption}: We train a CNN on Fashion MNIST in the i.i.d setting in presence of scaled bit flip corruption of stochastic gradients. Similar to Figure~\ref{figure:fmnist.image_corr}, \textsc{BGmD} achieves up to $\sim 3\times x$ speedup over \textsc{GmD} while being robust. For high corruption $\%$, \textsc{CmD} converges to sub-optimal solution.}}
\label{figure:fmnist.grad_corr}
% \vspace{-5mm} 
\end{figure}

\textbf{Corruption Simulations.} 
We consider three sources of error: corruption in \textbf{features}, corruption in \textbf{labels}, and corruption in \textbf{communicated gradients}. All the experiments are repeated for 0\% (i.e. clean), 10\%, 20\% and 40\% corruption levels, i.e, $\psi = 0, 0.1, 0.2, 0.4$, respectively (see Definition~\ref{definition:byzantine}).  
Below we describe three different perturbation models to simulate these real world corruptions.

\textbf{(a) Feature Corruption:} Here we consider corruption in the raw training data itself which can arise from different issues related to data collection. Particularly, adopting the corruptions introduced in \cite{hendrycks2018benchmarking}, we use two noise models to directly apply to the corrupt samples: \textit{(i) Additive}: Gaussian noise $\vz_i \sim \mathcal{N}(0 , 100)$ directly added to the image, and \textit{(ii) Impulse}: Salt and Pepper noise added by setting 90\% of the pixels to 0 or 1.

\textbf{(b) Gradient Corruption:}
In distributed training over multiple machines the communicated gradients  can be noisy, e.g., due to hardware issues or simply because some nodes are adversarial and aim to maliciously disrupt the training.
%%%%%%%%%%%
\setlength{\intextsep}{0pt}%
\setlength{\columnsep}{6pt}%
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-5pt}
\centering
\subfloat{\includegraphics[width=0.22\textwidth]{figs/grad_viz/clean_viz.png}}
\subfloat{\includegraphics[width=0.22\textwidth]{figs/grad_viz/45_viz.png}}
\caption{\label{figure:robust_gar_val} \footnotesize{\textbf{Gradient Corruption}: Left: No Corruption, Right: 45 \% gradients corrupted with additive Gaussian noise. This Toy example visually demonstrates the superior robustness properties of \textsc{Gm} for robust mean estimation (e.g. estimating the aggregated gradient)}}
\end{wrapfigure}
%%%%%%%%%%%
Using standard noise models for gradient corruption~\cite{fu1998penalized, xie2019zeno, bernstein2018signsgd} we directly corrupt the gradients in the following manner:
\textit{(i) Additive}: adversary adds random Gaussian noise $\vz_i \sim \mathcal{N}(0, 100)$ to the true gradient, and
\textit{(ii) Scaled Bit Flip}: corrupted gradients $\vg_t^{c}$ are  the scaled bit flipped version of the true gradient estimate; in particular, we use the following scale: $\vg_t^c = - 100 \vg_t$. % \textbf{(iii) Sign Flip}: adversary randomly flips the sign of 70\% co-ordinates \cite{bernstein2018signsgd}. 

\textbf{(c) Label Corruption:} We simulate the important real world backdoor attack~\cite{shen2019learning, tolpegin2020data}where the goal of the adversary is to bias the classifier towards some adversary chosen class. To simulate this at each iteration we flip the labels of randomly chosen $\psi$ fraction of the samples to a \textbf{target} label (e.g. in Fashion MNIST we use 8:bag as the backdoor label). 


\textbf{Dynamic Corruption Strategy.}
In order to represent a wide array of real world adversarial scenarios we use the following dynamic corruption strategy: At each iteration, we randomly sample $\psi$ fraction of the samples malicious. Note that this implies none of the samples are trustworthy and thus makes the robust estimation problem truly unsupervised
\footnote{This is a strictly stronger and realistic simulation of corruption compared to existing literature where a fixed set of samples are treated as malicious throughout the training.}. % implying in some rounds it is possible to not have any outlier samples whereas our strategy ensures that at each iteration we are presented with $\alpha-$ corruption set. 

\textbf{Discussion on the Test Performance.}
In Table~\ref{table:fmnist_table} we observe that without corruption both \textsc{BgmD} and \textsc{GmD} are able to achieve similar accuracy as the baseline (i.e., \textsc{SGD}). Conversely, \textsc{CmD} has a significant sub-optimality gap even in the clean setting. We observe the same trend under different corruption models over various levels of corruption. When corruption is high, \textsc{SGD} starts to diverge  after a few iterations. While \textsc{CmD} doesn't diverge, at higher level of corruptions its performance significantly degrades. On the other hand, both \textsc{GmD} and \textsc{BGmD} remain robust and maintain their test accuracy as expected from thier strong theoretical guarantees. Surprisingly, \textbf{\textsc{BGmD} not only maintains similar robustness as \textsc{GmD}, in several experiments it even outperforms} the performance of \textsc{GmD}. We hypothesize that this might be because of implicit regularization properties of \textsc{BGmD} in over-parameterized settings. 

\setlength{\intextsep}{0pt}%
\setlength{\columnsep}{3pt}%
\begin{wrapfigure}{r}{0.36\textwidth}
\centering
\includegraphics[width=0.36\textwidth]{figs/neurips/role_k.png}
\caption{\label{figure:choice_k}\footnotesize{\textsc{BGMD} with different values of $k$ and with / without memory on MNIST using CNN demonstrating the importance of memory augmentation}}
\vspace{-2mm}
\end{wrapfigure}
\textbf{Discussion on the Relative Speedup.} 
The main goal of this work is to speed up \textsc{Gm} based robust optimization methods. To this end, we verify the efficiency of different methods via plotting the performance on test set as a function of the \textbf{wall clock time}. Figure~\ref{figure:fmnist.image_corr} and Figure~\ref{figure:fmnist.grad_corr} suggest that under a variety of corruption settings \textsc{BgmD} is able to achieve significant speedup over \textsc{GmD} often by more than 3x while maintaining a similar test performance.

\textbf{Choice of $k$ and the Role of Memory.} In order to study the importance the memory mechanism we train a 4-layer CNN on MNIST~\cite{lecun1998gradient} dataset while retaining $0<\beta \leq 1$ fraction of  coordinates, i.e., $k = \beta d$. Figure~\ref{figure:choice_k} shows that the training runs that used memory (denoted by M) were able to achieve a similar accuracy while using significantly fewer coordinates. 

The above empirical observations highlight the following insights: \textbf{(a)} For challenging corruption levels/models, \textsc{Gm} based methods are indeed superior while standard \textsc{SGD} or \textsc{CmD} can be significantly inaccurate, \textbf{(b)} In all of our reported experiments, \textsc{BGmD} was run with $k$ set to 10\% of the number of parameters. Despite using such a small ratio \textsc{BGmD} retains the strong performance of \textsc{GmD}. \textbf{(c)} By judiciously choosing $k$, \textsc{BGmD} is more efficient than \textsc{GmD}, and \textbf{(d)} memory augmentation is vital for \textsc{BGmD} to attain a high accuracy while employing relatively small values of $k$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[htb!]
\vspace{-3 mm}
\subfloat[Original Image]{\includegraphics[width=0.24\columnwidth]{figs/neurips/im_sample.png}}
\subfloat[Gaussian Noise]{\includegraphics[width=0.24\columnwidth]{figs/neurips/im_sample_gauss.png}}
\subfloat[Salt \& Pepper Noise]{\includegraphics[width=0.24\columnwidth]{figs/neurips/im_sample_sp.png}}
\subfloat[Gaussian Blur]{\includegraphics[width=0.24\columnwidth]{figs/neurips/im_sample_blur.png}}\\
\subfloat{\includegraphics[width=0.24\columnwidth]{figs/grad_viz/clean_viz.png}}
\subfloat{\includegraphics[width=0.24\columnwidth]{figs/grad_viz/10_viz.png}}
\subfloat{\includegraphics[width=0.24\columnwidth]{figs/grad_viz/30_viz.png}}
\subfloat{\includegraphics[width=0.24\columnwidth]{figs/grad_viz/45_viz.png}}
\caption{\small \textbf{Corruption in Feature}: We demonstrate the effect of perturbations added to the corrupt images}
\label{figure:robust_gar_val}
\end{figure}

\subsection{\textsc{\textbf{Experimental Details}}}
\vspace{-1.5 mm}
In all the experiments, we compare both convergence rates (training loss) as well as generalization performance (test accuracy). 
All models are trained using 4 NVIDIA Tesla V100 GPUs, each pairing 5,120 CUDA Cores and 640 Tensor Cores exploiting Data Parallelism \cite{tarditi2006accelerator}. We used categorical cross entropy loss with $\ell_2$ regularization with weight decay value of 1e-4 across all experiments and a common learning rate schedule: learning rate is reduced by $1\%$ after each epoch. In particular, we perform the following three representative experiments to demonstrate robustness and convergence of \textsc{BgmD} across different training paradigm. 

(A) \textit{\textbf{Single Batch Training}}\\
We trained a LeNet\cite{lecun1998gradient} on Fashion-MNIST \cite{xiao2017fashion} in simple \textit{vanilla batch setting} with batch size of 128 and initial learning rate of 0.01. In (Figure \ref{figure:fmnist.lenet}) we plot the convergence and accuracy under different levels of \textit{Additive Corruption}. For this setting, \textsc{BGmD} was run with block size $k = 0.05 \times d$ where $d$ is total number of parameters in LeNet.  

(B) \textit{\textbf{Distributed Mini Batch Training}}\\
For the second setting, we trained a ResNet-18 \cite{he2016deep} on CIFAR-10 \cite{krizhevsky2012imagenet} in a distributed mini-batch setting with 20 parallel mini-batches each with a batch size of 128. In this setting; note that unlike robust aggregation happened over the communicated batch gradients instead of sample gradients. Figure \ref{figure:distributed.cifar.resnet} shows the training and generalization performance of under \textit{\textbf{Random Corruption}}. Using a block size equal to 5\% of the total parameters \textsc{BGmD} was able to match the performance of \textsc{Gm-SGD}.

(C) \textit{\textbf{Federated Training}}\\
For this experiment we consider a two-layer neural network(NN) with ReLU activation, each layer 300 neurons wide. We train this NN in a Federated Learning setting where 20 local clients each with access to a different shard of data collaboratively learn the objective in conjunction with a server node. 
 
To simulate heterogeneous (non i.i.d) data distribution among clients we use the following scheme:  \textit{The entire training data was first sorted based on labels and then divided into 80 equal data-shards $\gD_i$ i.e. for Fashion-MNIST each data shard was assigned 750 samples. Further this implies that each shard can have at most data from 2 class labels \footnote{Since each class has 6000 samples and the shards are sampled contiguously in a label sorted manner implies that each shard has only 1 class label with probability 7/8 and at most 2 class labels with probability 1/8.}. Each client was then randomly assigned \hl{4} shards of data implying each client had access to \hl{4} classes on an average.} 

Further, the clients only \textit{communicated periodically} with the server after every 10 rounds of local steps. The communicated gradients were further quantized to 2 bits before communicating to the server using $\mathrm{qsgd}$ \cite{alistarh2017qsgd} as given below: 
\begin{equation*}
	\mathrm{qsgd}_b(\vx) = \frac{\mathrm{sign}(\vx)\|\vx\|}{2^{b}w}\left\lfloor2^{b}\frac{|\vx|}{\|\vx\|}+u\right\rfloor, \quad \mathrm{qsgd}_b(\mathbf{0}) = \mathbf{0}
\end{equation*}
For \textsc{BGmD} we used block size \hl{$k = 0.1 \times d$}. Figure \ref{figure:federated.mlp.fmnist} shows the empirical results under this setting\footnote{Due to lack of space, we only show a subset of our results in the main paper. A more complete set of experiments can be found in the supplementary material.}

\subsection{\textsc{\textbf{Discussion}}} 
\vspace{-1.5 mm}
The key takeaways from the experiments are: \\
\textbullet \; \textit{\textbf{Convergence}}. From the results, it can be seen that \textsc{BGmD} converges at a comparable rate to \textsc{Gm-SGD} in all three settings strengthening our theoretical findings. \\
\textbullet \; \textit{\textbf{Generalization and Robustness:}} These experiments reveal that under both clean and corrupt settings, 
settings \textsc{BGmD} is able to match or even outperform \textsc{Gm-SGD}.  \\
\textbullet\; \textit{\textbf{Value of k:}} One important question remains: \textit{what should be a good value of k}?  As suggested in Proposition \ref{proposition:compute}, by choosing smaller $k$ we could achieve considerable speedup over \textsc{Gm-SGD}. However, in our experiments we found that while for larger models (LeNet , ResNet) by choosing $k$ in the order of 5\% of the parameter dimension, we are able to achieve strong results however, for the smaller 2 layer NN, such small value of $k$ would lead to slow convergence in spite of the error feedback mechanism, dwarfing the speedup from \textsc{BGmD}. This is potentially because of inherent sparsity patterns in the larger models due to over parameterization. 

% This is possibly depends on the structure (sparsity pattern, low rank) of the problem. As a consequence of over-parameterization, large scale deep learning models are often likely to have sparse structure \cite{shi2019understanding} allowing for even more aggressive choice of $k$. %likely to have extremely sparse gradient estimates \cite{shi2019understanding}. 
%\centering
%\subfloat[No Corruption]{\includegraphics[width=0.5\columnwidth]{figs/icml/effect_k.png}\label{figure:k_clean}}
%\subfloat[$10\%$ Corruption]{\includegraphics[width=0.5\columnwidth]{figs/icml/effect_k_noise.png}\label{figure:k_noisy}}
%\label{}
%\caption{\footnotesize Convergence of \textsc{BGmD} for different values of $k$}
%\vspace{-4mm}
%\end{figure}

\end{comment}


==> fed_bgmd.tex <==
\input{arxiv/fed_bgmd_algo_block}
In this section we extend \textsc{BGmD} to the task of federated learning (FL) \cite{mcmahan2017communication} setting which we will refer as \textsc{Fed-BgmD} hereafter. 
The full algorithm summarized in Algorithm \ref{algorithm:full.fl}. \\*[0.2cm]
\textbf{(Periodic Communication).} Given that in the FL setting the clients communicate with the cloud only periodically, they store their current local models in rounds where they perform local gradient updates using a new variable $\vy_t^i$ which is set to the global model $\vx_t$ whenever there is a communication round $t\in \gI_T$, e.g., every $H$ iteration (Assumption \ref{assumption:period}). \\*[0.2cm]
\textbf{(Communication Compression).} In each communication round, the clients communicate a compressed gradient estimate $c_t^i\gQ(\vx_t-\vy_{t+0.5}^i)$ which is approximated as the compressed difference between the last global model $\vx_t$ and the current local model $\vy_{t+0.5}^i$ (by taking a gradient step). Intuitively, this difference is the accumulated local gradients multiplied by the step size, hence we expect it to become small as the training progresses. Here, we assume $\gQ(.)$ is an unbiased randomized quantization (Definition \ref{definition:quantization}) operator satisfying $\E\|\gQ(\vx)-\vx\|^2\leq q\|\vx\|^2$. For example, the qsgd operator \cite{alistarh2017qsgd} satisfies this condition. \\*[0.2cm]
\textbf{(Global Model Update).}The global model update at the central server is relatively similar to that of \textsc{BGmD} where in each communication round we employ memory and $\epsilon$-accurate \textsc{Gm} to perform the update and find the next model $\vx_{t+1}$ which will be communicated to the clients.
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lemma:qsparse}
Let, $\mG_t^\ast$ denote the gradient matrix with each row corresponding to uncompressed gradient estimates then we claim that Algorithm \ref{algorithm:full.fl} yields the following contraction approximation: 
\begin{equation*}
    \E_{\gC_k} \left[\|\gC_k(\mG_t)-\mG_t^\ast\|_F^2 |\vx\right] \leq (1-\xi)\|\mG_t^\ast\|_F^2 \quad , \quad  (1 - \beta_{k,s})\frac{k}{d} \leq \xi \leq 1
\end{equation*}
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> fed_bgmd_algo_block.tex <==
\textcolor{blue}{
\begin{algorithm}[!htb]
	\caption{FL-\textsc{BGmD}}
	\label{algorithm:full.fl}
	\algsetup{indent=2em}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} 
		stepsize $\gamma$, number of iterations $T$, synchronization rounds $\gI_T$, accuracy of the \textsc{Gm} oracle $\{\epsilon\}_{t=0}^{T-1}$; \vspace{1mm}
		\STATE {\bfseries initialize:} $\vx_0 = \vx_0^i = \vy_0^i$, $\vm_0^i = \mathbf{0}$ for all $i\in [n]\backslash \sB$ \vspace{1mm}
		\FOR{ $t =0,\dots, T-1$}
		\STATE \textbf{On Clients:}\vspace{1mm}
		\FOR{$i =1,\dots, n$ in parallel}\vspace{1mm}
		\IF {$i\in \sG$ }\vspace{1mm}
		\STATE $\vg_t^i = \nabla F_i(\vy_t^i,z_t^i)\quad$ (computing the local stochastic gradient $\vg_t^i$)\vspace{1mm}
		\STATE $\vy_{t+0.5}^i = \vy_{t}^i-\gamma \vg_t^i\quad $ (local first-order update)\vspace{1mm}
		\IF {$ t+1 \not\in \gI_T$}\vspace{1mm}
		\STATE $\vx_{t+1} =\vx_t,$ $\vy_{t+1}^i = \vy_{t+0.5}^i\quad$ (updating only the local model) \vspace{1mm} 
		\ELSE
			\STATE $\vc_t^i = \gQ(\vx_t-\vy_{t+0.5}^i) $ (sending the message $\vc_t^i$ to the server)\vspace{1mm}
		\STATE $\vy_{t+1}^i = \vx_{t+1}\quad $(receive the aggregated model from the server)\vspace{1mm}
		\ENDIF
		\ELSE
		\STATE $\vg_t^i = \square, \quad \vc_t^i= \blacksquare ,\quad \forall i\in \sB\quad $ (arbitrary  messages) \vspace{1mm}
		\ENDIF
		\ENDFOR
		\STATE \textbf{At Server:}\vspace{1mm}
		\IF {$ t+1 \not\in \gI_T$}\vspace{1mm}
		\STATE $\vx_{t+1} =\vx_t,\quad$ (no updates to the global model)\vspace{1mm}
		\ELSE
		        \STATE     $\mG_t \in \sR^{n \times d}$ s.t. $\mG[i, :] = \vc_t^i$\vspace{1mm}
            \STATE $\mP_t:= \gamma_t\mG_t + \mM_t^s$ \quad (server error correction)\vspace{1mm}
            \STATE $\boldsymbol{\Delta}_t := \gC_k(\mG_t)$ \quad (Run Algorithm \ref{algorithm:co_sparse_approx})\vspace{1mm}
           \STATE  $\mM_{t+1}^s := \mP_t - \boldsymbol{\Delta}_t $ \quad (update server residual)\vspace{1mm}
            \STATE $\Tilde{\vg}_t := \textsc{Gm}(\epsilon,\boldsymbol{\Delta}_t)$ \quad(Robust Aggregation in $\sR^k$)\vspace{1mm}
           \STATE $\vx_{t+1}:= \vx_t - \Tilde{\vg}_t$ \quad (Global model update)\vspace{1mm}
		\ENDIF
		\ENDFOR
	\end{algorithmic}
\end{algorithm}
}

==> intro_v2.tex <==
Consider smooth non-convex optimization problems with finite sum structure: 
\begin{equation}
    \label{equation:finite_sum}
    \min_{\mathbf{x}\in \R^d} \left[\bar{f}(\mathbf{x}):=\frac{1}{n}\sum_{i=1}^n f_i(\mathbf{x})\right]
\end{equation}
Mini-batch SGD is the de-facto method for optimizing such functions \cite{robbins1951stochastic, bottou2010large, tsitsiklis1986distributed} which proceeds as follows: at each iteration $t$, it selects a random batch $\gD_t$ of $b$ samples, obtains gradients $\vg_t^{(i)}=\nabla f_i(\vx_t), \quad \forall i \in \gD_t$ and updates the parameters using iterations of the form: 
\begin{equation}
\label{equation:sgd}
\vx_{t+1} := \vx_t - \gamma \Tilde{\vg}^{(t)} ,\quad 
\Tilde{\vg}^{(t)} = \frac{1}{|\gD_t|} \sum_{i\in \gD_t} \vg_i^{(t)}
\end{equation}
In spite of its strong convergence properties in the standard settings \cite{moulines2011non, dekel2012optimal, li2014efficient, goyal2017accurate, keskar2016large, yu2012large}, it is well known that even a small fraction of corrupt samples can lead SGD to an arbitrarily poor solution \cite{bertsimas2011theory, ben2000robust}. 
This has motivated a long line of work to study robust optimization in presence of corruption [\textcolor{red}{citations}].
While the problem has been studied under a variety of contamination models, in this paper we study the robustness properties of first-order methods \eqref{equation:sgd} under the strong and practical \textbf{gross contamination model} (See Definition~\ref{definition:byzantine}) \cite{li2018principled, diakonikolas2019recent, diakonikolas2019sever, diakonikolas2019robust} which also \textit{generalizes the popular Huber's contamination model and the byzantine contamination framework} \cite{huber1992robust, lamport1982byzantine}. In particular, the goal of this work is to design an {\em efficient} first order optimization methods to solve ~\eqref{equation:finite_sum}, that remains {\em robust} even when $0 \leq \psi < 1/2$ fraction of the gradient estimates $\vg_t^{(i)}$ are \textit{arbitrarily corrupted} in each batch $\gD_t$ \textbf{without any prior knowledge about the malicious samples}.   

% That is, the goal is to design an {\em efficient} and {\em robust} optimization method that can tolerate $\alpha$-fraction of corrupted gradients under \textbf{gross contamination model} \cite{li2018principled, diakonikolas2019recent, diakonikolas2019sever, diakonikolas2019robust} in each batch $\gD_t$. Robustness of a method is measured by it's breakdown point --- largest fraction of contamination that must be introduced to cause an estimator to break (see Definition~\ref{assumption:breakdown_point}). 
% \paragraph{\bf Robust \textsc{SGD} via \underline{G}eometric \underline{M}edian \underline{D}escent (\textsc{GmD})}
Under the gross corruption model, the vulnerability of mini-batch SGD can be attributed to the linear gradient aggregation employed in \eqref{equation:sgd} \cite{blanchard2017machine, alistarh2018byzantine, yin2018byzantine, xie2019zeno}. In fact, \textit{no linear gradient aggregation strategy} can tolerate even a \textit{single} grossly corrupted update, i.e.,  they have a \textit{breakdown point} (Definition \ref{assumption:breakdown_point}) of 0. \footnote{To see this, consider the following single malicious gradient  $\vg_t^{(j)} = -\sum_{i \in {\gD_t \setminus j}}\vg_t^{(i)}$ which implies that the average becomes $\mathbf{0}$, hence SGD would be stuck at the initialization.}  
%\paragraph{\bf Robust \textsc{SGD} via \underline{G}eometric \underline{M}edian \underline{D}escent (\textsc{GmD})}
%\subsection{Robust \textsc{SGD} via \underline{G}eometric \underline{M}edian \underline{D}escent (\textsc{GmD})}
%Under the strong corruption model (Definition \ref{definition:byzantine}), the vulnerability of mini-batch SGD can be attributed to the linear gradient aggregation employed in \eqref{equation:sgd} \cite{blanchard2017machine, alistarh2018byzantine, yin2018byzantine, xie2019zeno}. In fact, it can be shown that \textit{no linear gradient aggregation strategy} can tolerate even a \textit{single} grossly corrupted update, i.e.,  they have a \textit{breakdown point} (Definition \ref{assumption:breakdown_point}) of 0. To see this, consider the following single malicious gradient  $\vg_t^{(j)} = -\sum_{i \in {\gD_t \setminus j}}\vg_t^{(i)}$. Then, one can see that this single corrupted gradient results in the average to become $\mathbf{0}$, which in turn means mini-batch SGD getting stuck at the initialization.
%The above arguments motivate the study of robust estimation, where the goal is to find an estimate $\Tilde{g}$ over $\alpha$-corrupted set $\gD_t$ such that with high probability $\| \Tilde{g} - \frac{1}{\sG} \sum_{\vg_i \in \sG} \vg_i\|$ is small. Also note that this would imply that the solution of \eqref{equation:finite_sum} in presence of $\alpha$-corruption is close to the true solution \eqref{equation:true_f}. We refer the reader to \cite{diakonikolas2019recent} and references therein for a comprehensive discussion on unsupervised robust mean estimation. 
That is, despite the presence of outliers, the goal would be to estimate the {\em true} mean of the correct gradients . For this problem, geometric median (\textsc{Gm}) (Definition \ref{assumption:geo_med}) is a popular robust estimator  with \textbf{optimal breakdown point} of $\frac{1}{2}$ even in gross corruption model \cite{lopuhaa1991breakdown,feng2014distributed,minsker2015geometric}. Hence, it has been used extensively to make SGD robust with several papers studying the breakdown point and convergence rate \cite{alistarh2018byzantine, chen2017distributed, pillutla2019robust, wu2019federated}.


%In this context, geometric median (\textsc{Gm}) (Definition \ref{assumption:geo_med}) is known to be a rotation and translation invariant robust mean estimator which \textit{achieves the \textbf{optimal breakdown point} of $\frac{1}{2}$ even in the presence of gross corruption} \cite{lopuhaa1991breakdown,feng2014distributed,minsker2015geometric}. Simply put, \textsc{Gm} remains a good estimator of the true mean of the good samples even when up to half of the samples are \textit{arbitrarily corrupted} \cite{cohen2016geometric}. Due to this strong robustness property of \textsc{Gm}, SGD  with  \textsc{Gm}-based gradient aggregation (\textsc{Gm-SGD}) becomes robust even under a gross corruption model \cite{alistarh2018byzantine, chen2017distributed, pillutla2019robust, wu2019federated}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Despite the strong robustness guarantees of \textsc{Gm}, the computational cost of calculating \textsc{Gm} is prohibitive, especially in high dimensional settings, and has attracted considerable attention \cite{vardi2000multivariate,weiszfeld1937point,chandrasekaran1989open,chin2013runtime,cohen2016geometric,pillutla2019robust}. For example, \cite{cohen2016geometric} provides an $\epsilon$-approximate \textsc{Gm} estimator with $O(d/\epsilon^2)$ computational operations. Despite these efforts, in practical large-scale optimization settings, such as training deep learning models where the number of parameters ($d$) is extremely large (e.g.,  $d \approx 60M$ for AlexNet, $d \approx 175B$ for GPT-3), \textsc{Gm} remains prohibitively expensive to compute \cite{chen2018draco, pillutla2019robust} limiting it's applicability. 
%scaling the challenge remains and all the known methods to compute an approximate \textsc{Gm} solution, scale poorly with the dimension  of the problem ($d$) \cite{cohen2016geometric, pillutla2019robust, diakonikolas2019recent, diakonikolas2019robust}.  Thus, in practical large-scale optimization settings, such as the task of training deep learning models where the number of parameters ($d$) is extremely large (e.g.,  $d \approx 60M$ for AlexNet, $d \approx 175B$ for GPT-3), \textsc{Gm} remains prohibitively expensive to compute \cite{chen2018draco, pillutla2019robust}, limiting the practicality of \textsc{Gm-SGD} and its variants to small-scale settings.


\paragraph{Robust \textsc{SGD} via \underline{G}eometric \underline{M}edian \underline{D}escent (\textsc{GmD})}
In this work we design a new method based on a memory augmented block coordinate selection strategy (Algorithm \ref{algorithm:co_sparse_approx}) which can significantly reduce the computational overhead of \textsc{Gm} based gradient aggregation and leads to nearly {\em two orders of magnitude} speedup over existing robust optimization techniques for standard deep learning training tasks, while maintaining almost the same level of accuracy.


At a high level, our algorithm (\textsc{BGmD}) selects a block of $ 0 < k \leq d$ {\em important} coordinates of the gradients; importance of a coordinate is measured according to the largest directional derivative measured by the squared $\ell_2$ norm across all the samples (Algorithm \ref{algorithm:co_sparse_approx}). The remaining $(d-k)$ dimensions are discarded and gradient aggregation happens only along these selected $k$ directions. So, the geometric median (\textsc{Gm}) is computed over gradient vectors in $\sR^k$ (a lower dimensional subspace) only. Thus, when $k\ll d$, this approach provides a practical solution to deploy \textsc{Gm}-based aggregation in high dimensional settings\footnote{The notation $k\ll d$ implies that $k$ is at least an order of magnitude smaller than $d$}. 

The motivation behind reducing the \textit{dimension} of the gradient vectors is that in many scenarios most of the information in the gradients is captured by a subset of the coordinates. Hence, by the judicious block coordinate selection subroutine outlined in Algorithm \ref{algorithm:co_sparse_approx} we are able to identify an informative low-dimensional representation of the gradients.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%. Overview of Algorithm 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Overview of Our Algorithm}
%Assume we are given a \textit{black-box} $\epsilon$-approximate \textsc{Gm} oracle (see Definition \ref{assumption:geo_med}). \textit{The main goal of this work is to modify the iterates of \textsc{Gm}-based robust \textsc{SGD} in a way such that even in high dimensional settings the resultant first-order iterates have a total computational cost comparable with vanilla mini-batch \textsc{SGD} with linear averaging \eqref{equation:sgd} while maintaining similar robustness properties as \textsc{Gm-SGD} in the gross corruption setting}. 

%To this end, we propose the \textsc{B}lock co-ordinate \textsc{Gm} \textsc{D}escent (\textsc{BGmD}) method (Algorithm \ref{algorithm:full}) which proceeds as follows: %\footnote{Anonymized Code Available: \href{https://anonymous.4open.science/r/f0788f17-4b66-4cff-afdc-034de41c3cff/}{Link}}
%at each iteration, a set $\gD_t=\{i_1, \dots, i_b\}$ of $b$ samples is chosen; the corresponding stochastic gradients $\vg_t^{(i)} = \nabla f_i(\vx_t) \in \sR^d, \; \forall i \in \gD_t$ are obtained using an unbiased oracle (Assumption \ref{assumption:bounded_g}). At this point,
%we select a block of $ 0 < k \leq d$ coordinates according to the largest directional derivative measured by to the squared $\ell_2$ norm across all the samples (Algorithm \ref{algorithm:co_sparse_approx}). The remaining $(d-k)$ dimensions are discarded and gradient aggregation happens only along these selected $k$ directions. This procedure implies that the \textsc{Gm} based gradient aggregation sub-routine operates on $n$ gradient vectors in $\sR^k$ (a lower dimensional subspace) and by imposing $k\ll d$ this approach provides a practical solution to deploy \textsc{Gm}-based aggregation in high dimensional settings\footnote{The notation $k\ll d$ implies that $k$ is at least an order of magnitude smaller than $d$}. 

%The motivation behind reducing the \textit{dimension} of the gradient vectors is that in many scenarios most of the information in the gradients is captured by a subset of the coordinates. Hence, by the judicious block coordinate selection subroutine outlined in Algorithm \ref{algorithm:co_sparse_approx} we are able to identify an informative low-dimensional representation of the gradients.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{arxiv/algo_block}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% As we discuss thoroughly in our experiments, although 
While algorithm \ref{algorithm:co_sparse_approx} identifies a representative block of the coordinates; \textbf{aggressively reducing the dimension} (i.e., $k\ll d$) might lead to a significant approximation error, which in turn might lead to slower convergence (i.e., more iterations), dwarfing the benefit from reduction in per iteration compute \cite{nesterov2012efficiency, nutini2015coordinate}. To alleviate this, leveraging the idea of Error Compensation \cite{seide20141}, in Algorithm \ref{algorithm:full} we introduce \textit{memory augmentation}. Specifically, at each iteration the residual error from dimensionality reduction is computed and stored in memory i.e., $\mM_t$ and in the subsequent iteration, this memory $\mM_t$ is added back to the new gradient estimates. Our ablation studies show that such memory augmentation indeed ensures that the number of iterations remain relatively small. 

\paragraph{Contributions.} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The main contributions of this work are as follows: 
\vspace{-2mm}
\begin{itemize}\setlength \itemsep{0.05em}
\item We propose \textsc{BGmD} (Algorithm \ref{algorithm:full}); a method for robust optimization in large-scale high dimensional settings % with  the optimal breakdown point of 1/2 
that results in  significant savings in the computational costs compared to \textsc{Gm}-SGD while maintaining optimal breakdown point 1/2. To the best of our knowledge, \textsc{BGmD} is the first method that can maintain similar high breakdown point as \textsc{Gm}-SGD while attaining strong convergence guarantees and significantly reduced per iteration compute; making it an attractive choice for robust optimization in high dimensions.

\item Our proposed approach also highlights the following key insight: \textit{In the context of robust optimization, performing robust gradient estimation in a low dimensional subspace has little to no impact in the downstream optimization task especially in case of over-parameterized models.} Thus, by judiciously selecting a block of co-ordinates and performing robust mean estimation only in this low-dimensional subspace is a practical approach to leverage highly robust estimators like \textsc{Gm} even in high dimensional setting which was previously intractable (scaling poorly with dimension). In Algorithm \ref{algorithm:co_sparse_approx} we also propose a simple strategy for selecting the block of coordinates.  

\item In addition to the proposed coordinate selection procedure, we also introduce a memory mechanism that allows us to aggressively select very few coordinates (thus resulting in huge savings in computation per iteration) while maintaining convergence properties (taking similar number of iterations to converge) comparable to  \textsc{Gm}-SGD. 
 
% To the best of our knowledge this is the first work to robustly train SGD in presence gross corruption with optimal breakdown point of 1/2 ; while using the same compute SGD** 
% We propose an algorithm to make GM based robust SGD feasible in high dimensional settings. We do Block CD. 
% To the best of our knowledge this is the first computationally tr Gm based 
% \item ** To the best of our knowledge this is the first work to adapt an error compensation mechanism to block co-ordinate descent to improve the convergence. ** 
%\item Distributed learning susceptible to faults in various nodes. Faults are hard to characterize, so best to assume worst case faults. 
%\item For standard distributed SGD, this implies that gradients from some of the nodes can be arbtirary corrupted. 
%\item Existing literature has shown that geometric median can solve this problem well, i.e.,  it can get good solution despite presence of a few faults. 
%\item But computing geometric median is computationally challening, and the best known methods either need d/eps2 or ndlog1/eps computation. That is, the method scales poorly wrt dimensionality.
%\item We propose sampling coordinates of gradient on which geometric median is performed. 
%\item But even without geometric median, coordinate descent might perform poorly.
%\item So, we combine sampling with error feedback technique. The key intution is that geometric median in general can be much more expensive than computing error feedback. So overall the algorithm is significantly less expensive. 
\item We provide strong guarantees on the rate of convergence of \textsc{BGmD} in standard non-convex scenarios including smooth non-convex functions, and non-convex functions satisfying the Polyak-\L{}ojasiewicz Condition. These rates are comparable to those established for \textsc{Gm}-SGD under more restricting conditions such as strong convexity \cite{ chen2017distributed,pillutla2019robust,wu2019federated}.
% , and show that for certain error level, the method is indeed more efficient than the existing robust FL methods (bartlett, pittula+kakade). \textcolor{red}{Note that our results are quite general. Our rates are derived under periodic communication and does not make any i.i.d assumption. Implying, our rates apply to full federated learning setting with heterogeneous client distribution, periodic communication and partial device participation (See Section \ref{section:discussion}). We also extend our algorithm and theoretical results in case of unbiased compressed communication (ex. quantization).}
\item \textcolor{red}{Elaborate More} Through extensive %deep learning 
experiments under several common corruption settings; we demonstrate that \textsc{BGmD} can achieve significant speedup with respect the \textsc{Gm}-SGD while achieving nearly the same training and test performance 
%(i.e. robustness).  
% Our experiments are even more surprising, where we show that the method actually converges to a better error rate than even standard robust FL. and is significantly more efficient. \textcolor{red}{We use Fashion MNIST - LeNet ; CIFAR10 - VGG , SST2 (NLP) - wordCNN}
% \item * Also note that several other algorithms ex. Krum with strong robustness guarantees also scales poorly with dimension. While in this paper we present the algorithm and analyze in the context of GM - we would like to point out that our proposed scheme is more general and can also be 
%%%%% Commented for NeuRips %%%%%%% 
\begin{comment}
\item We further develop and analyze an extension of \textsc{BGmD} to federated learning (FL) - a new distributed optimization paradigm \cite{mcmahan2017communication}. We call this algorithm \textsc{Fed-BGmD}. We also provide convergence guarantees for \textsc{Fed-BGmD} under smooth non-convex and non-convex objective with PLC. Our theoretical results are general and holds under compressed periodic communication over heterogeneous client data distribution. 
% and  We also demonstrate its efficacy in several robust FL tasks. 
\end{comment}

\end{itemize}


TO BE MOVED TO PRELIMINARIES: 
In this paper we study the robustness properties of first-order methods \eqref{equation:sgd} under the following strong \textbf{gross contamination model} \cite{li2018principled, diakonikolas2019recent, diakonikolas2019sever, diakonikolas2019robust} which also \textit{generalizes the popular Huber's contamination model and the byzantine contamination framework} \cite{huber1992robust, lamport1982byzantine}. In particular, we assume that an $\psi$ fraction  of the gradient estimates $\vg_t^{(i)}$ can be \textit{arbitrarily corrupted} (Definition \ref{definition:byzantine}),
and study the convergence properties of (robustified) first-order methods to solve \eqref{equation:finite_sum} \textit{without any prior knowledge about the malicious samples}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}[{\textbf{Gross Corruption Model}}]
\label{definition:byzantine}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Given $0 \leq \psi < \frac{1}{2}$ and a distribution family $\gD$ on $\sR^d$ the adversary operates as follows: $n$ samples are drawn from $D \in \gD$. The adversary is allowed to \textbf{inspect} all the samples and replace up to $\psi n$ samples with arbitrary points. 

\textup{Intuitively, this implies that $(1 - \psi)$ fraction of the training samples are generated from the true distribution (\textit{inliers}) and rest are allowed to be \textbf{arbitrarily corrupted} (\textit{outliers}) i.e. $\alpha:=|\sB|/ |\sG|= \frac{\psi}{1 - \psi} < 1$, where $\sB$ and $\sG$ are the sets of corrupt and good samples. In the rest of the paper, we will refer to a set of samples generated through this process as \bf{$\alpha$-corrupted}.}
\end{definition}
Also note that, by letting the corrupt estimates to be \textit{arbitrarily skewed}, this corruption model is able to capture a number of (if not all) important practical scenarios including existence of outliers, software bugs, hardware failure, numerical errors arising from commodity hardware, or unreliable communication channels during distributed or federated training and also black-box adversarial attack scenarios \cite{chen2017targeted,liao2018backdoor, gu2019badnets, biggio2012poisoning, mhamdi2018hidden,tran2018spectral}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}[{\textbf{Breakdown Point}}]
\label{assumption:breakdown_point}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In robust statistics, 
Finite-sample breakdown point \textup{\cite{donoho1983notion}} is a way to measure the resilience of an estimator. It is defined as the largest fraction of contamination that must be introduced to cause an estimator to break i.e. produce arbitrarily wrong estimates.

\textup{In the context Definition \ref{definition:byzantine} we can say an estimator has the optimal breakdown point 1/2 if it is robust in presence of $\alpha$-corruption $\forall \; \psi < 1/2$ or alternatively $\forall \; \alpha < 1$}.
\end{definition}

% (See Assumption \ref{assumption:byzantine}), commonly referred to as \textit{gross corruption} \cite{li2018principled} or the 
% also referred as the \textit{Byzantine generals framework} \cite{lamport1982byzantine}. 

%In particular, we assume that an $\alpha$ fraction  of the gradient estimates $\vg_t^{(i)}$ can be \textit{arbitrarily corrupted} (Assumption \ref{assumption:byzantine}),
% and study the convergence properties of (robustified) first-order methods to solve \eqref{equation:finite_sum} \textit{without any prior knowledge about the malicious samples}. 
% Note that, by letting the corrupt estimates to be \textit{arbitrarily skewed}, this corruption model is able to capture a number of important practical scenarios including existence of outliers, software bugs, hardware failure, numerical errors arising from commodity hardware, or unreliable communication channels during distributed or federated training and also black-box adversarial attack scenarios \cite{chen2017targeted,liao2018backdoor, gu2019badnets, biggio2012poisoning, mhamdi2018hidden,tran2018spectral}.


%\subsection{Outline}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}[{\textbf{Geometric Median}}]
\label{assumption:geo_med}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Given a finite collection of observations $\vx_1, \vx_2, \dots \vx_n$ defined over 
a separable Hilbert space $\mathbb{X}$ with norm $\|\cdot\|$ the geometric median or the Fermet-Weber point is defined as \textup{\cite{haldane1948note,weber1929alfred,minsker2015geometric,kemperman1987median}}
\begin{equation}
\label{equation:gm}
    \vx_* = \textsc{Gm}(\{\vx_i\}) =\argmin_{\vy\in \mathbb{X}} \bigg[g(\vx):=\sum_{i=1}^{n}\|\vy - \vx_i\|\bigg]
\end{equation}
We call a point $\vx \in \R^d$ an $\epsilon$-accurate geometric
median if $g(\vx) \leq (1+\epsilon)g(\vx_*)$
% If $\mu$ is a probability measure on Banach space $\mathbb{X}$ with norm $\|\cdot\|$ then the geometric median (\textsc{Gm}) or the Fermet-Wever point is defined as \cite{haldane1948note, weber1929alfred, minsker2015geometric}
%\begin{equation}
%    \vx_* = \argmin_{\vy \in \mathbb{X}} %\int_{\mathbb{X}}(\|\vy-\vx\|-\|\vx\|)\mu(dx)
%\end{equation}
%For all the analysis in this work we will restrict ourselves to the special case when $\mathbb{X}$ is a separable Hilbert space $\mathbb{H}$ and $\mu$ is the empirical measure of finite points $\vx_1, \vx_2, ... , \vx_n \in \mathbb{X}$. It is also worth noting, that in this special case the operator \textsc{Gm}$(\cdot)$ is unique as long as as all $\vx_i$ don't lie on the same line \cite{kemperman1987median}.
%\begin{equation}
%    \vx_* = \argmin_{\vy\in \mathbb{X}} \sum_{i=1}^{n}\|\vy - \vx_i\|
%\end{equation}
\end{definition}


==> proof_fed_bgmd.tex <==
\section{Proof of Lemma \ref{lemma:qsparse}}
\begin{proof}
First we note that, during each communication round i.e for all iterations $t \in \gI_T$ the clients communicate quantized (Definition \ref{definition:quantization}) stochastic gradient estimates to the server in order to reduce the communication overhead. This implies that $i$ th row of $\mG_t$ in the server of Algorithm \ref{algorithm:full.fl} can be written as: $\mG_t[i, :] = \gQ(\vg_t^i)$. Let the corresponding gradient jacobian with true stochastic gradients be $\mG_t^\ast$ where: $\mG_t^\ast[i, :] = \vg_t^i$. Now note that by applying block sampling as described in Algorithm \ref{algorithm:co_sparse_approx} , for each row we yield a \textbf{composition} of compression. Now, we can use Lemma 1 of \cite{basu2019qsparse} in conjunction with our Lemma \ref{lemma:norm_sampling} to get the desired result.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\section{Detailed Statements of the Theorems}
\newtheorem*{theorem3*}{Theorem \ref{theorem:non_convex_simple.fl}}
\begin{theorem3*}
[\textbf{Smooth Non-convex}]
Suppose Assumptions \ref{assumption:byzantine}--\ref{assumption:compression},\ref{assumption:period} specified in Section \ref{section:prelim} hold. For any stepsize $\gamma := 1/2L$, after $T$ iterations the iterates of Algorithm \ref{appendix:algorithm_fl} satisfy with
\begin{equation}
\label{eq:thm:nonconvex-FL}
\begin{aligned}
\frac{1}{T|\sG|} \sum_{t=0}^{T-1}\sum_{i\in\sG}&\text{ }\E\|  \nabla f(\vy_t^i)\|^2 \leq \frac{8(f(\vx_0)-f^\ast)}{\gamma T}+8L\gamma\sigma^2+24 L^2 \gamma^2H^2\sigma^2\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]
\\
&+ \frac{2304 |\gI_T|H^2\sigma^2}{T(1-\alpha)^2}\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]+\frac{48|\gI_T|\epsilon^2}{\gamma^2T|\sG|^2(1-\alpha)^2}.
    \end{aligned}
\end{equation}
\end{theorem3*}

\newtheorem*{theorem4*}{Theorem \ref{theorem:plc_simple.fl}}
\begin{theorem4*}
[\textbf{Non-convex under PLC}]
Suppose Assumptions \ref{assumption:byzantine}--\ref{assumption:plc} specified in Section \ref{section:prelim} hold. For any step size $\gamma := 1/4L$, after $T$ iterations the iterates of Algorithm \ref{appendix:algorithm_fl} satisfy
\begin{equation}
\label{equation:thm:plc}
\begin{aligned}
\frac{1}{|\sG|}\sum_{i\in\sG} &\text{ }\E\|\hat{\vy}_T^i-\vx^\ast\|^2 \leq \frac{16(f(\vx_0)-f^\ast)}{\mu^2\gamma}\left[1-\frac{\mu\gamma}{2}\right]^T\\&+\frac{16L\gamma\sigma^2}{\mu^2}+\frac{40 L^2}{\mu^2} \gamma^2H^2\sigma^2\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]\\
&+\frac{3072 H^2\sigma^2}{\mu^2(1-\alpha)^2}\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]+\frac{64\epsilon^2}{\mu^2\gamma^2 |\sG|^2(1-\alpha)^2},
 \end{aligned}
 \end{equation}
 for a global optimal solution  $\vx^\ast \in \gX^\ast$. Here,
 $\hat{\vy}_T^i := \frac{1}{W_T}\sum_{t=0}^{T-1}w_t\vy_t^i$ with weights $w_t := (1-\frac{\mu\gamma}{2})^{-(t+1)}$, $W_T := \sum_{t=0}^{T-1}w_t$.
%  where $w_t = (1-\frac{\mu\gamma}{2})^{-(t+1)}$, $W_T = \sum_{t=0}^{T-1}w_t$, and $\vq^i_t \in \gX^\ast$, for all $i\in \sG$ and $t=0,\dots T-1$.
\end{theorem4*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Intermediate Lemmas}
Before proving Theorem \ref{theorem:non_convex_simple.fl} and Theorem \ref{theorem:plc_simple.fl} we prove several necessary intermediate lemmas. These lemmas can be thought of as the extensions of those used in the proofs of Theorem \ref{theorem:nonconvex-simple} and Theorem \ref{theorem:plc-simple} by noting the consideration that in the FL setting the clients communicate with the server periodically. To this end, we also define: 
\begin{equation}
    \vy_t = \sum_{i\in\sG} \vy_t^i,\quad 
\end{equation}
\begin{equation}
    \tilde{\vy}_{t+1}^i = \tilde{\vy}_{t}^i - \gamma \vg_t^i -\sI\{t+1\in\gI_T\}\vz_t, \quad \tilde{\vy}_{0}^i = \vy_0^i = \vx_0,
\end{equation}
and the average virtual sequence
\begin{equation}
\begin{aligned}
    \tilde{\vy}_{t+1}&= \frac{1}{|\sG|}\sum_{i\in \sG}\tilde{\vy}_{t+1}^i \\& = \tilde{\vy}_{t}- \gamma \vg_t -\sI\{t+1\in\gI_T\}\vz_t,
    \end{aligned}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[\bf Variation of \textsc{Gm}-based update]
\label{lemma:bound-z}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Consider the setting of Algorithm \ref{algorithm:full.fl} in iteration $t$ with tolerance parameter $\epsilon \geq 0$, compression factor $\xi$ (Lemma \ref{lemma:qsparse}). Then in presence of $\alpha-$corruption (Definition \ref{definition:byzantine}) under Assumption \ref{assumption:period} and Assumption \ref{assumption:bounded_g} it holds that: 
\begin{equation}
\label{equation:bound-z}
    \E\|\vz_t\|^2 \leq \frac{96\gamma^2H^2\sigma^2}{(1-\alpha)^2}\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]+\frac{2\epsilon^2}{|\sG|^2(1-\alpha)^2}.
\end{equation}
\end{lemma}

\begin{proof}
The proof is a generalization of Lemma \ref{lemma:bound-z-simplified}. Since $\Tilde{\vg}_t$ is the $\epsilon$-accurate \textsc{Gm} of $\{\Delta_t^i\}_i$, 
% $\vz_t$ can be thought of as the $\epsilon$-accurate \textsc{Gm} of $\{\Delta_t^i-\Delta_t\}_i$. Thus, by the classical robustness property of \textsc{Gm} (Theorem. 2.2 in \cite{lopuhaa1991breakdown}; see also \cite{minsker2015geometric,cohen2016geometric,chen2017distributed,li2019rsa,wu2019federated} for similar adaptations) we have
\begin{equation}
\label{equation:bound-z0}
    \E\|\vz_t\|^2\leq \frac{8|\sG|}{(|\sG|-|\sB|)^2}\sum_{i\in \sG}\E\|\Delta_t^i-\Delta_t\|^2+\frac{2\epsilon^2}{(|\sG|-|\sB|)^2}.
\end{equation}
Next, we bound $\E\|\Delta_t^i-\Delta_t\|^2$ using the properties of memory mechanism stated in Lemma \ref{lemma:bound-e}. To this end, we may write:
\begin{equation}
\label{equation:bound-z1}
\begin{aligned}
  \E\|\Delta_t^i-\Delta_t\|^2&= 2\E\|\Delta_t^i\|^2+2\E\|\Delta_t\|^2 \\&\leq 2\E\|\Delta_t^i\|^2+\frac{2}{|\sG|}\sum_{i\in \sG}\E\|\Delta_t^i\|^2\\&\leq
  4\max_{i\in \sG}\E\|\Delta_t^i\|^2,
  \end{aligned}
\end{equation}
where we used Fact \ref{fact:1} twice. Next, we establish a bound on the norm of the communicated messages as follows. Add add and  subtract $\vp_t^i$ and use the update rule of the memory to obtain
\begin{equation}
\label{equation:bound-z2}
\begin{aligned}
  \E\|\Delta_t^i\|^2&= \E\|\Delta_t^i+\vp_t^i-\vp_t^i\|^2 \\&= \E\|\vp_t^i-\vm_{t+1}^i\|^2\\&=\E\|\vx_t-\vy_{t+0.5}^i+\vm_{t}^i-\vm_{t+1}^i\|^2\\&\leq 3\E\|\vx_t-\vy_{t+0.5}^i\|^2+3\E\|\vm_{t}^i\|^2+3\E\|\vm_{t+1}^i\|^2,
  \end{aligned}
\end{equation}
by definition of $\vp_t^i$ and Fact \ref{fact:1}. Notice that using Lemma \ref{lemma:bound-e} we can uniformly bound the last two terms on the RHS of \eqref{equation:bound-z2}:
\begin{equation}\label{equation:bound-z22}
\begin{aligned}
  3\E\|\vm_{t}^i\|^2+3\E\|\vm_{t+1}^i\|^2 \leq \frac{24(1-\xi^2)\gamma^2H^2\sigma^2}{\xi^2}.
  \end{aligned}
\end{equation}
Thus, to establish an upper bound on  $\E\|\Delta_t^i\|^2$ it remains to bound the first term. To do this, note that $\vx_t$ is the latest global update received by node $i$ from the server at a communication round that we may denote by $\tau \in \gI_T$ such that $\tau \leq t$. That is, $\vx_t = \vx_\tau$. Additionally, once $\vx_\tau$ is received each client updates its local variable to this global update, i.e., $\vy_\tau^i=\vx_\tau$. Now, given the local first-order update adapted in Algorithm \ref{algorithm:full} it holds that 
\begin{equation}
\label{equation:bound-z3}
  \vy_i^t = \vy_\tau^i - \gamma \sum_{\ell=\tau}^{t-1} \vg_\ell^i. 
\end{equation}
Consequently, 
\begin{equation}
\label{equation:bound-z4}
\begin{aligned}
    \E\|\vx_t-\vy_{t+0.5}^i\|^2 &= \E\|\vx_\tau-\vx_\tau+\gamma \sum_{\ell=\tau}^{t-1} \vg_\ell^i\|^2\\&=\gamma^2\E\|\sum_{\ell=\tau}^{t-1} \vg_\ell^i\|^2\\&\leq \gamma^2(t-\tau)\sum_{\ell=\tau}^{t-1}\E\| \vg_\ell^i\|^2\\&\leq \gamma^2H^2\max_{\tau\leq\ell<t}\E\| \vg_\ell^i\|^2\\&\leq
    \gamma^2H^2\sigma^2,
    \end{aligned}
\end{equation}
where we used Fact \ref{fact:1}, the Assumption that the two consecutive global updates are not more than $H$ iterations apart, and the bounded SFO assumption. Therefore, we conclude
\begin{equation}\label{equation:bound-z5}
\begin{aligned}
\E\|\Delta_t^i\|^2&\leq3\gamma^2H^2\sigma^2+\frac{24(1-\xi^2)\gamma^2H^2\sigma^2}{\xi^2}.
    \end{aligned}
\end{equation}
Therefore, by \eqref{equation:bound-z1} and \eqref{equation:bound-z5}
\begin{equation}
\label{equation:bound-z6}
\begin{aligned}
  \E\|\Delta_t^i-\Delta_t\|^2& \leq 12\gamma^2H^2\sigma^2\left[1+\frac{4(1-\xi^2)}{\xi^2}\right],
  \end{aligned}
\end{equation}
and the proof is complete by combining this last result with \eqref{equation:bound-z0}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[\textbf{Induced Delay of the Local Models}]
\label{lemma:bound-virtual}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Consider the setting of Algorithm \ref{algorithm:full.fl} in iteration $t$. It holds that:
\begin{equation}
\label{equation:bound-virtual}
 \vy_t - \tilde{\vy}_t = \vm_t.
\end{equation}
\end{lemma}
\begin{proof}
Due to periodic communication, we cannot use Lemma \ref{lemma:bound-virtual-simplified} directly. To generalize Lemma \ref{lemma:bound-virtual-simplified}, we start by noting that there exists  $\ell+1\in\gI_T$, $\ell+1\leq t$, such that
\begin{equation}\label{equation:bound-virtual:1}
  \vy_t - \tilde{\vy}_t = \vy_{\ell+1} - \tilde{\vy}_{\ell+1} 
\end{equation}
This relation obviously holds with $\ell=t-1$ if $t\in \gI_T$, i.e., $t$ is a communication round. Assume the largest $\ell$ such that $\ell+1 < t$, $\ell+1\in\gI_T$, and $t\not\in \gI_T$. Then, from the definitions of $\vy_t $ and $ \tilde{\vy}_t$ we know
\begin{equation}
\label{equation:bound-virtual:2}
    \vy_t = \vy_{\ell+1}-\gamma \sum_{j=\ell+1}^{t-1}\vg_j,\quad \tilde{\vy}_t = \tilde{\vy}_{\ell+1}-\gamma \sum_{j=\ell+1}^{t-1}\vg_j-\sum_{j=\ell+1}^{t-1}\sI\{j+1\in\gI_t\}\vz_j.
\end{equation}
However, it is evident that for all $j\in\{\ell+1,\dots,t-1\}$, $j+1\not\in\gI_T$. Thus, noting \eqref{equation:bound-virtual:2} we establish \eqref{equation:bound-virtual:1}. Now, we derive again find a recursive relation for the difference $\vy_{\ell+1} - \tilde{\vy}_{\ell+1} $ for the iterations that clients communicate with the server.
Let $q+1<\ell+1$ be the previous communication round. Due to aggregation at $\ell+1$ we have $\vy_{\ell+1} = \vx_{\ell+1}$. Thus, by the server update
\begin{equation}
\label{equation:bound-virtual:3}
\begin{aligned}
    \vy_{\ell+1} &= \vx_\ell-\Tilde{\vg}_\ell \\&= \vx_\ell - \Delta_\ell-\vz_\ell.
    \end{aligned}
\end{equation}
On the other hand,
\begin{equation}
\label{equation:bound-virtual:4}
\begin{aligned}
    \tilde{\vy}_{\ell+1} &= \tilde{\vy}_{q+1} -\gamma \sum_{j=q+1}^{\ell}\vg_j  -\gamma \sum_{j=q+1}^{\ell}\sI\{j+1\in\gI_t\}\vz_j \\&=\tilde{\vy}_{q+1} -\gamma \sum_{j=q+1}^{\ell}\vg_j -\vz_\ell \\&=\tilde{\vy}_{q+1}-(\vy_{q+1}-\vy_{\ell+0.5})-\vz_\ell,
    \end{aligned}
\end{equation}
where we used the fact that there is no communication between $q+1$ and $\ell+1$ iterations and  the update of the local models, i.e., $\vy_t^i$'s. Collectively, \eqref{equation:bound-virtual:3} and \eqref{equation:bound-virtual:4} imply
\begin{equation}
\label{equation:bound-virtual:5}
\begin{aligned}
    \vy_{\ell+1} - \tilde{\vy}_{\ell+1} &=(\vy_{q+1} - \tilde{\vy}_{q+1})+(\vx_\ell-\vy_{\ell+0.5}-\Delta_\ell).
    \end{aligned}
\end{equation}
Since $\vy_{0} =\tilde{\vy}_{0}$ using induction yields
\begin{equation}
\label{equation:bound-virtual:6}
\begin{aligned}
    \vy_{\ell+1} - \tilde{\vy}_{\ell+1} &=\sum_{j+1\in\gI_T,j\leq \ell}(\vx_j-\vy_{j+0.5}-\Delta_j)\\&=\sum_{j+1\in\gI_T,j\leq \ell}(\vm_{j+1}-\vm_j)\\&=\vm_{\ell+1}-\vm_0\\&=\vm_{t},
    \end{aligned}
\end{equation}
where we used the fact that $\vm_0=\mathbf{0}$ and the memory variables remain unchanged between two consecutive communication rounds. The proof is complete by noting  \eqref{equation:bound-virtual:1}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[\textbf{Variation of the Local Models}]
\label{lemma:bound-variation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Consider the setting of Algorithm \ref{algorithm:full.fl} in iteration $t$ with compression factor $\xi$ (Lemma \ref{lemma:qsparse}). Then in presence of $\alpha-$corruption (Definition \ref{definition:byzantine}), under Assumption \ref{assumption:bounded_g},\ref{assumption:period} it holds that:
\begin{equation}
    \E\|\tilde{\vy}_{t}-\vy_t^i\|^2 \leq 2\gamma^2H^2\sigma^2\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]
\end{equation}
\end{lemma}
\begin{proof}
Using Fact \ref{fact:1} we may write
\begin{equation}
\label{equation:lemma:bound-variation1}
\begin{aligned}
\E\|\tilde{\vy}_{t}-\vy_t^i\|^2 &\leq 2\E\|\tilde{\vy}_{t}-\vy_t\|^2+2\E\|\vy_t-\vy_t^i\|^2\\
&= 2\E\|\vm_t\|^2+2\E\|\vy_t-\vy_t^i\|^2,
    \end{aligned}
\end{equation}
where we applied Lemma \ref{lemma:bound-virtual}. The memory in \eqref{equation:lemma:bound-variation1} can be dealt with using the result of Lemma \ref{lemma:bound-e}. On the other hand, recall
\begin{equation}
\label{equation:lemma:bound-variation2}
\begin{aligned}
\vy_t &= \frac{1}{|\sG|}\sum_{i\in\sG}\vy_t^i\\
&= \frac{1}{|\sG|}\sum_{i\in\sG} \vy_\tau^i -\gamma \sum_{j=\tau}^{t-1} \vg_j^i\\
&= \frac{1}{|\sG|}\sum_{i\in\sG} \vy_\tau -\gamma \sum_{j=\tau}^{t-1} \vg_j^i\\
&=  \vy_\tau -\gamma \sum_{j=\tau}^{t-1} \vg_j,
    \end{aligned}
\end{equation}
where $\tau\in \gI_T$, $\tau\leq t$ is the previous communication round. Thus,
\begin{equation}
\label{equation:lemma:bound-variation3}
\begin{aligned}
\E\|\vy_t-\vy_t^i\|^2 &= \E\|(\vy_t^i-\vy_\tau^i)-(\vy_t-\vy_\tau)\|^2\\
&\leq \E\|\vy_t^i-\vy_\tau^i\|^2\\
&\leq \E\|\gamma \sum_{j=\tau}^{t-1} \vg_j^i\|^2\\
&\leq \gamma^2(t-\tau)\sum_{j=\tau}^{t-1}\E\|\vg_j^i\|^2\\
&\leq \gamma^2H^2\sigma^2,
    \end{aligned}
\end{equation}
using Fact \ref{fact:1}, Assumption \ref{assumption:bounded_g}, and  fact that two consecutive global updates are not more than $H$ iterations apart. The proof is complete by this result and noting \eqref{equation:lemma:bound-variation1} while using Lemma \ref{lemma:bound-e}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem \ref{theorem:non_convex_simple.fl}}
We first consider the setting of smooth non-convex functions.
\begin{proof}
Recall that $\vg_t = \frac{1}{|\sG|}\sum_{i\in\sG}\nabla F_i(\vy_t^i,z_t^i)$. By the definition of $L$-smoothness (see Assumption \ref{assumption:smooth}), we have
\begin{equation}
\label{equation:thm:1}
\begin{aligned}
    f(\tilde{\vy}_{t+1}) &\leq f(\tilde{\vy}_{t})+ \langle \nabla f(\tilde{\vy}_{t}), \tilde{\vy}_{t+1}-\tilde{\vy}_{t}\rangle+\frac{L}{2}\|\tilde{\vy}_{t+1}-\tilde{\vy}_{t}\|^2\\
    &= f(\tilde{\vy}_{t})+ \langle \nabla f(\tilde{\vy}_{t}), -\gamma \vg_t-\sI\{t+1\in\gI_T\}\vz_t\rangle+\frac{L}{2}\|\gamma \vg_t+\sI\{t+1\in\gI_T\}\vz_t\|^2\\
    &\leq f(\tilde{\vy}_{t}) -\gamma \langle \nabla f(\tilde{\vy}_{t}),  \vg_t \rangle -\langle\nabla f(\tilde{\vy}_{t}),\sI\{t+1\in\gI_T\}\vz_t\rangle+L\gamma^2\| \vg_t\|^2\\&\qquad\qquad+L\|\sI\{t+1\in\gI_T\}\vz_t\|^2.
    \end{aligned}
\end{equation}
Let $\E_t$ denote expectation with respect to sources of randomness in computation of stochastic gradients at the clients at time $t$. Then,
\begin{equation}
\label{equation:thm:2}
\begin{aligned}
\E_t[f(\tilde{\vy}_{t+1})] &\leq f(\tilde{\vy}_{t})-\gamma \langle \nabla f(\tilde{\vy}_{t}),  \bar{\vg}_t \rangle -\sI\{t+1\in\gI_T\}\E_t[\langle\nabla f(\tilde{\vy}_{t}),\vz_t\rangle]+L\gamma^2\E_t\| \vg_t\|^2\\&\qquad\qquad+\sI\{t+1\in\gI_T\}L\E_t\|\vz_t\|^2.
 \end{aligned}
 \end{equation}
 The first inner-product in \eqref{equation:thm:2} can be bounded according to
 \begin{equation}
 \label{equaton:thm:3}
\begin{aligned}
2\langle \nabla f(\tilde{\vy}_{t}),  \bar{\vg}_t \rangle &= \|\nabla f(\tilde{\vy}_{t})\|^2 + \|\bar{\vg}_t\|^2-\|\nabla f(\tilde{\vy}_{t})-  \bar{\vg}_t\|^2\\
 &\geq  \|\nabla f(\tilde{\vy}_{t})\|^2 -\|\nabla f(\tilde{\vy}_{t})-  \bar{\vg}_t\|^2\\
&= \|\nabla f(\tilde{\vy}_{t})\|^2 -\| \frac{1}{|\sG|}\sum_{i\in\sG}\nabla f_i(\tilde{\vy}_{t})-  \frac{1}{|\sG|} \sum_{i\in\sG} \nabla f_i(\vy_t^i)\|^2\\
&\geq \|\nabla f(\tilde{\vy}_{t})\|^2 -\frac{1}{|\sG|}\sum_{i\in\sG}\| \nabla f_i(\tilde{\vy}_{t})-  \nabla f_i(\vy_t^i)\|^2\\
&\geq \|\nabla f(\tilde{\vy}_{t})\|^2 -\frac{L^2}{|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}-  \vy_t^i\|^2\\
&= \|\nabla f(\tilde{\vy}_{t})\|^2 +\frac{L^2}{|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}-  \vy_t^i\|^2-\frac{2L^2}{|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}-  \vy_t^i\|^2\\
&\geq \|\nabla f(\tilde{\vy}_{t})\|^2 +\frac{1}{|\sG|}\sum_{i\in\sG}\|\nabla f(\tilde{\vy}_{t})-  \nabla f(\vy_t^i)\|^2-\frac{2L^2}{|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}-\vy_t^i\|^2\\
&= \frac{1}{|\sG|}\sum_{i\in\sG}\|\nabla f(\tilde{\vy}_{t})\|^2 +\frac{1}{|\sG|}\sum_{i\in\sG}\|\nabla f(\tilde{\vy}_{t})-  \nabla f(\vy_t^i)\|^2-\frac{2L^2}{|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}-\vy_t^i\|^2\\
&\geq  \frac{1}{2|\sG|}\sum_{i\in\sG}\|  \nabla f(\vy_t^i)\|^2-\frac{2L^2}{|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}-\vy_t^i\|^2,
 \end{aligned}
 \end{equation}
 where we employed  Fact \ref{fact:1} and $L$-smoothness of each local function several times. Therefore, 
  \begin{equation}\label{equation:thm:1inner}
\begin{aligned}
-\gamma\langle \nabla f(\tilde{\vy}_{t}),  \bar{\vg}_t \rangle \leq -\frac{\gamma}{4|\sG|} \sum_{i\in\sG}\|  \nabla f(\vy_t^i)\|^2+\frac{\gamma L^2}{|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}-\vy_t^i\|^2.
 \end{aligned}
 \end{equation}
 We now bound the second inner-product. To this end,
 \begin{equation}\label{equation:thm:2inner}
 \begin{aligned}
     -\E_t[\langle\nabla f(\tilde{\vy}_{t}),\vz_t\rangle] &= -\E_t[\langle \frac{1}{|\sG|}\sum_{i\in\sG}\nabla f(\vy_t^i),\vz_t\rangle]+\E_t[\langle\frac{1}{|\sG|}\sum_{i\in\sG}\nabla f(\vy_t^i)-\nabla f(\tilde{\vy}_{t}),\vz_t\rangle]\\
     &\leq \frac{\rho\gamma}{|\sG|} \sum_{i\in\sG}\|  \nabla f(\vy_t^i)\|^2+\frac{1}{2\rho\gamma}\E_t\|\vz_t\|^2+\E_t[\langle\frac{1}{|\sG|}\sum_{i\in\sG}\nabla f(\vy_t^i)-\nabla f(\tilde{\vy}_{t}),\vz_t\rangle]\\
     &\leq\frac{\rho\gamma}{2|\sG|} \sum_{i\in\sG}\|  \nabla f(\vy_t^i)\|^2+\frac{1}{2\rho\gamma}\E_t\|\vz_t\|^2+\frac{1}{2\gamma}\E_t\|\vz_t\|^2\\&\qquad\qquad+\frac{\gamma}{2|\sG|}\sum_{i\in\sG}\|\nabla f(\vy_t^i)-\nabla f(\tilde{\vy}_{t})\|^2\\
     &\leq\frac{\rho\gamma}{2|\sG|} \sum_{i\in\sG}\|  \nabla f(\vy_t^i)\|^2+\left(\frac{1}{2\rho\gamma}+\frac{1}{2\gamma}\right)\E_t\|\vz_t\|^2+\frac{\gamma L^2}{2|\sG|}\sum_{i\in\sG}\|\vy_t^i-\tilde{\vy}_{t}\|^2,
      \end{aligned}
 \end{equation}
 where we used Fact \ref{fact:2} twice and to obtain the last inequality we employed the smoothness assumption. Here, $0<\rho<0.5$ is a parameter whose value will be determined later.
 
Application of \eqref{equation:thm:1inner} and \eqref{equation:thm:2inner} in  \eqref{equation:thm:2} yields
\begin{equation}
\label{equation:thm:4}
\begin{aligned}
\E_t[f(\tilde{\vy}_{t+1})] &\leq f(\tilde{\vy}_{t})-\left(\frac{1}{2}-\rho\right)\frac{\gamma}{2|\sG|} \sum_{i\in\sG}\|  \nabla f(\vy_t^i)\|^2+\frac{3\gamma L^2}{2|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}-\vy_t^i\|^2\\
&\qquad\qquad+L\gamma^2\E_t\|\vg_t\|^2+\sI\{t+1\in\gI_T\}\left(L+\frac{1}{2\rho\gamma}+\frac{1}{2\gamma}\right)\E_t\|\vz_t\|^2.
    \end{aligned}
\end{equation}
Rearranging and taking expectation with respect to the entire sources of randomness, i.e., the proposed coordinated sparse approximation method and the randomness in computation of stochastic gradient in iterations $0,\dots,t-1$, as well as the bounded SFO assumption yields 
\begin{equation}
\label{equation:thm:5}
\begin{aligned}
\left(\frac{1}{2}-\rho\right)\frac{\gamma}{2|\sG|}& \sum_{i\in\sG}\E\|  \nabla f(\vy_t^i)\|^2 \leq \E[f(\tilde{\vy}_{t})]-\E[f(\tilde{\vy}_{t+1})]+\frac{3\gamma L^2}{2|\sG|}\sum_{i\in\sG}\E\|\tilde{\vy}_{t}-\vy_t^i\|^2\\
&\qquad\qquad+L\gamma^2\sigma^2+\sI\{t+1\in\gI_T\}\left(L+\frac{1}{2\rho\gamma}+\frac{1}{2\gamma}\right)\E\|\vz_t\|^2.
    \end{aligned}
\end{equation}
Evidently, we need to bound two quantities in \eqref{equation:thm:5}. Lemma \ref{lemma:bound-z} establishes a bound on $\E\|\vz_t\|^2$ while Lemma \ref{lemma:bound-variation} deals with $\E\|\tilde{\vy}_{t}-\vy_t^i\|^2$.
Thus,
\begin{equation}
\label{equation:thm:6}
\begin{aligned}
\left(\frac{1}{2}-\rho\right)&\frac{\gamma}{2|\sG|} \sum_{i\in\sG}\E\|  \nabla f(\vy_t^i)\|^2 \leq \E[f(\tilde{\vy}_{t})]-\E[f(\tilde{\vy}_{t+1})]+L\gamma^2\sigma^2\\
&\qquad+\frac{3\gamma L^2}{2} 2\gamma^2H^2\sigma^2\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]
\\
&\qquad+\sI\{t+1\in\gI_T\}\left(L+\frac{1}{2\rho\gamma}+\frac{1}{2\gamma}\right) \frac{96\gamma^2H^2\sigma^2}{(1-\alpha)^2}\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]\\
&\qquad+\sI\{t+1\in\gI_T\}\left(L+\frac{1}{2\rho\gamma}+\frac{1}{2\gamma}\right)\frac{2\epsilon^2}{|\sG|^2(1-\alpha)^2}.
    \end{aligned}
\end{equation}
Finally, let $\rho = 1/4$ and $\gamma = \frac{1}{2L}$. We obtain the stated result by averaging \eqref{equation:thm:6} over time and noting $f^\ast\leq\E[f(\tilde{\vy}_{T})]$ and $f(\tilde{\vy}_{0}) = f(\vx_0)$. 
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem \ref{theorem:plc_simple.fl}}
\begin{proof}
Recall \eqref{equation:thm:5} in the proof of Theorem \ref{theorem:non_convex_simple.fl}. Let $a_{t} :=\E[f(\tilde{\vy}_{t})] -f^\ast \geq 0$. Using Assumption \ref{assumption:plc} to bound the gradient terms in \eqref{equation:thm:5} yields
\begin{equation}\label{equation:thm:plc1}
\begin{aligned}
a_{t+1} &\leq a_t - \left(\frac{1}{2}-\rho\right)\frac{\gamma\mu}{|\sG|} \sum_{i\in\sG}\E[f(\vy_t^i)-f^\ast]+\frac{3\gamma L^2}{2|\sG|}\sum_{i\in\sG}\E\|\tilde{\vy}_{t}-\vy_t^i\|^2\\
&\qquad\qquad+L\gamma^2\sigma^2+\sI\{t+1\in\gI_T\}\left(L+\frac{1}{2\rho\gamma}+\frac{1}{2\gamma}\right)\E\|\vz_t\|^2.
    \end{aligned}
\end{equation}
The above result is not sufficient to complete the proof since $a_{t}$ is with respect to the virtual sequence. 
% This difficulty, which is addressed for the first time in this paper,  has been the main challenge in the proof of convergence of error compensated schemes with biased gradient compression under PLC. 
To deal with this burden, we revisit \eqref{equation:thm:2} to establish an alternative bound. Specifically, we to bound the first inner-product in \eqref{equation:thm:2} we instead establish
\begin{equation}
\label{equation:thm:plc2}
\begin{aligned}
-\gamma \langle \nabla f(\tilde{\vy}_{t}),  \bar{\vg}_t \rangle &= -\gamma \langle \nabla f(\tilde{\vy}_{t}),  \nabla f(\tilde{\vy}_{t}) \rangle+\gamma \langle \nabla f(\tilde{\vy}_{t}),  \nabla f(\tilde{\vy}_{t})-\bar{\vg}_t \rangle\\
&\leq -\gamma\| \nabla f(\tilde{\vy}_{t})\|^2+\frac{\gamma\rho_1}{2}\| \nabla f(\tilde{\vy}_{t})\|^2+\frac{\gamma}{2\rho}\|\nabla f(\tilde{\vy}_{t})-\bar{\vg}_t\|^2\\
&= -\gamma(1-\frac{\rho_1}{2})\| \nabla f(\tilde{\vy}_{t})\|^2+\frac{\gamma}{2\rho_1}\|\nabla f(\tilde{\vy}_{t})-\bar{\vg}_t\|^2,
    \end{aligned}
\end{equation}
where we used Fact \ref{fact:2} with parameter $\rho_1>0$ which will be determined later. Recall that we already know how to bound $\|\nabla f(\tilde{\vy}_{t})-\bar{\vg}_t\|^2$ from the results established in \eqref{equation:thm:plc3}. That is,
\begin{equation}
\label{equation:thm:plc3}
\begin{aligned}
\|\nabla f(\tilde{\vy}_{t})-\bar{\vg}_t\|^2\leq\frac{L^2}{|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}- \vy_t^i\|^2.
 \end{aligned}
 \end{equation}
 We now derive a bound for the second inner-product in \eqref{equation:thm:2}. To do so, an application of Fact \ref{fact:2} yields 
 \begin{equation}
 \label{equation:thm:plc4}
\begin{aligned}
-\E_t[\langle\nabla f(\tilde{\vy}_{t}),\vz_t\rangle]\leq \frac{\rho_2\gamma}{2}\|\nabla f(\tilde{\vy}_{t})\|^2+\frac{1}{2\gamma\rho_2}\E_t\|\vz_t\|^2.
 \end{aligned}
 \end{equation}
 Therefore, in light of these new bounds we obtain
\begin{equation}
\label{equation:thm:plc5}
\begin{aligned}
\E_t[f(\tilde{\vy}_{t+1})] &\leq f(\tilde{\vy}_{t})-\gamma\left(1-\frac{\rho_1+\rho_2}{2}\right)\|\nabla f(\tilde{\vy}_{t})\|^2+L\gamma^2\E_t\| \vg_t\|^2\\
&+\sI\{t+1\in\gI_T\}\left(L+\frac{1}{2\gamma\rho_2}\right)\E_t\|\vz_t\|^2+\frac{\gamma L^2}{2\rho_1|\sG|}\sum_{i\in\sG}\|\tilde{\vy}_{t}- \vy_t^i\|^2.
 \end{aligned}
 \end{equation}
Subtracting $f^\ast$ and taking expectation with respect to the entire sources of randomness yields
\begin{equation}
\label{equation:thm:plc6}
\begin{aligned}
\E[f(\tilde{\vy}_{t+1})]-f^\ast &\leq \E[f(\tilde{\vy}_{t})]-f^\ast-\gamma\left(1-\frac{\rho_1+\rho_2}{2}\right)\E\|\nabla f(\tilde{\vy}_{t})\|^2+L\gamma^2\sigma^2\\
&+\sI\{t+1\in\gI_T\}\left(L+\frac{1}{2\gamma\rho_2}\right)\E\|\vz_t\|^2+\frac{\gamma L^2}{2\rho_1|\sG|}\sum_{i\in\sG}\E\|\tilde{\vy}_{t}- \vy_t^i\|^2.
 \end{aligned}
 \end{equation}
The gradient term $\E\|\nabla f(\tilde{\vy}_{t})\|^2$ in \eqref{equation:thm:plc6} can be related to $a_{t}$ using the PL condition. Therefore
\begin{equation}
\label{equation:thm:plc7}
\begin{aligned}
a_{t+1} &\leq \left[1-2\mu\gamma\left(1-\frac{\rho_1+\rho_2}{2}\right)\right]a_t+L\gamma^2\sigma^2\\
&+\sI\{t+1\in\gI_T\}\left(L+\frac{1}{2\gamma\rho_2}\right)\E\|\vz_t\|^2+\frac{\gamma L^2}{2\rho_1|\sG|}\sum_{i\in\sG}\E\|\tilde{\vy}_{t}- \vy_t^i\|^2.
 \end{aligned}
 \end{equation}
 Multiply \eqref{equation:thm:plc1} and \eqref{equation:thm:plc7} by $1/2$ and add the two to obtain
 \begin{equation}\label{equation:thm:plc8}
\begin{aligned}
a_{t+1} &\leq \left[1-\mu\gamma\left(1-\frac{\rho_1+\rho_2}{2}\right)\right]a_t+L\gamma^2\sigma^2-\left(\frac{1}{2}-\rho\right)\frac{\gamma\mu}{2|\sG|} \sum_{i\in\sG}\E[f(\vy_t^i)-f^\ast]\\
&\qquad+\sI\{t+1\in\gI_T\}\left(L+\frac{1}{4\gamma\rho}+\frac{1}{4\gamma\rho_2}+\frac{1}{4\gamma}\right)\E\|\vz_t\|^2\\
&\qquad+\left(3+\frac{1}{\rho_1}\right)\frac{\gamma L^2}{4|\sG|}\sum_{i\in\sG}\E\|\tilde{\vy}_{t}- \vy_t^i\|^2.
 \end{aligned}
 \end{equation}
 Define
 \begin{equation}\label{equation:thm:plc9}
     b_t := \frac{1}{|\sG|}\sum_{i\in\sG}\E[f(\vy_t^i)-f^\ast].
 \end{equation}
 Let $\rho=1/4$, $\rho_1=1/2$, $\rho_2=1/2$, and $\gamma = 1/4L$. Using Lemma \ref{lemma:bound-z} and Lemma \ref{lemma:bound-variation}, \eqref{equation:thm:plc8} simplifies to
\begin{equation}\label{equation:thm:plc10}
\begin{aligned}
a_{t+1} &\leq \left[1-\frac{\mu\gamma}{2}\right]a_t-\frac{\gamma\mu}{8} b_t+L\gamma^2\sigma^2+\frac{5 L^2}{2} \gamma^3H^2\sigma^2\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]\\
&\qquad+\left(\frac{192\gamma H^2\sigma^2}{(1-\alpha)^2}\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]+\frac{4\epsilon^2}{\gamma |\sG|^2(1-\alpha)^2}\right)\sI\{t+1\in\gI_T\}.
 \end{aligned}
 \end{equation}
 Thus, we can apply Fact \ref{fact:3} to obtain
 \begin{equation}
 \label{equation:thm:plc11}
\begin{aligned}
\frac{1}{W_T}\sum_{t=0}^{T-1}b_tw_t &\leq \frac{8(f(\vx_0)-f^\ast)}{\mu\gamma}\left[1-\frac{\mu\gamma}{2}\right]^T+\frac{8L\gamma\sigma^2}{\mu}+\frac{20 L^2}{\mu} \gamma^2H^2\sigma^2\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]\\
&+\frac{1536  H^2\sigma^2}{\mu(1-\alpha)^2}\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]+\frac{32}{\mu\gamma^2 |\sG|^2(1-\alpha)^2}\frac{\sum_{t=0}^{T-1}w_t\epsilon^2}{W_T},
 \end{aligned}
 \end{equation}
 where we used $E[f(\tilde{\vy}_0^i)] = f(\vx_0)$.
 Finally, to obtain the stated result we invoke Fact \ref{fact:4} and the assumption that the solution set (i.e., the set of all stationary points) is convex. Specifically, by the quadratic  growth condition and convexity of the Euclidean norm 
\begin{equation}
\label{equation:thm:plc12}
\begin{aligned}
\frac{1}{|\sG|}\sum_{i\in\sG}\sum_{t=0}^{T-1}\frac{w_t}{W_T}\E[f(\vy_t^i)-f^\ast] &\geq \frac{1}{|\sG|}\sum_{i\in\sG}\sum_{t=0}^{T-1}\frac{w_t}{W_T} \E\|\vy_t^i-\gP_{\gX^\ast}(\vy_t^i)\|^2\\
&\geq \frac{\mu}{2|\sG|}\sum_{i\in\sG}\sum_{t=0}^{T-1}\frac{w_t}{W_T} \E\|\vy_t^i-\gP_{\gX^\ast}(\vy_t^i)\|^2\\
&\geq \frac{\mu}{2|\sG|}\sum_{i\in\sG} \E\|\sum_{t=0}^{T-1}\frac{w_t}{W_T}\vy_t^i-\sum_{t=0}^{T-1}\frac{w_t}{W_T}\gP_{\gX^\ast}(\vy_t^i)\|^2\\
&:=\frac{\mu}{2|\sG|}\sum_{i\in\sG} \E\|\hat{\vy}_t^i-\vx^{\ast,i}_t\|^2,
 \end{aligned}
 \end{equation}
 where $\gP_{\gX^\ast}(\vy_t^i)$ is the projection of $\vy_t^i$ onto the solution set $\gX^\ast$ and $\vx^{\ast,i}_t:=\sum_{t=0}^{T-1}\frac{w_t}{W_T}\gP_{\gX^\ast}(\vy_t^i) \in \gX^\ast$ by the assumption that the solution set is convex.
\end{proof}

==> result_table_fmnist.tex <==
\begin{table}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}llllllllllllllll@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{SGD} & \multicolumn{3}{c}{BGMD} & \multicolumn{3}{c}{GMD} & \multicolumn{3}{c}{CMD}\\%\cmidrule(lr){1-1}
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
\textbf{Clean}    
& \multicolumn{3}{c}{$89.39\textcolor{gray}{\pm 0.28}$}   
& \multicolumn{3}{c}{$89.25 \textcolor{gray}{\pm 0.19}$}     
& \multicolumn{3}{c}{$88.98\textcolor{gray}{\pm 0.3}$}    
& \multicolumn{3}{c}{$83.82\textcolor{gray}{\pm 0.26}$} \\ %\midrule
\multicolumn{16}{c}{}  \\
Corruption (\%)         &\multicolumn{1}{c}{10}    &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}   &\multicolumn{1}{c}{10}    &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}    &\multicolumn{1}{c}{10}    &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}  &\multicolumn{1}{c}{10}    &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}\\\midrule

\multicolumn{16}{c}{Feature Attack}                         \\%\midrule
\multicolumn{16}{c}{}  \\
Additive 
%sgd
& \multicolumn{1}{c}{$45.52\textcolor{gray}{\pm 5.04}$} 
& \multicolumn{1}{c}{-} 
& \multicolumn{1}{c}{-}
%bgmd
& \multicolumn{1}{c}{$88.12\textcolor{gray}{\pm 0.55}$}
& \multicolumn{1}{c}{$86.76\textcolor{gray}{\pm 0.03}$} 
& \multicolumn{1}{c}{$82.27\textcolor{gray}{\pm 0.06}$}
%gmd
& \multicolumn{1}{c}{$88.12\textcolor{gray}{\pm 0.02}$}
& \multicolumn{1}{c}{$86.63\textcolor{gray}{\pm 0.04}$} 
& \multicolumn{1}{c}{$81.23\textcolor{gray}{\pm 0.03}$} 
%cmd
& \multicolumn{1}{c}{$83.12\textcolor{gray}{\pm 0.54}$}
& \multicolumn{1}{c}{$82.38\textcolor{gray}{\pm 0.13}$} 
& \multicolumn{1}{c}{$78.54\textcolor{gray}{\pm 0.65}$}
\\
Impulse    
%sgd
&\multicolumn{1}{c}{$83.82\textcolor{gray}{\pm 3.56}$}
&\multicolumn{1}{c}{$79.18\textcolor{gray}{\pm 6.47}$}  
&\multicolumn{1}{c}{-} 
%bgmd 
&\multicolumn{1}{c}{$88.21\textcolor{gray}{\pm 0.03}$}
&\multicolumn{1}{c}{$86.91\textcolor{gray}{\pm 0.36}$}  
&\multicolumn{1}{c}{$81.73\textcolor{gray}{\pm 0.06}$} 
%gmd
&\multicolumn{1}{c}{$88.19\textcolor{gray}{\pm 0.02}$}
&\multicolumn{1}{c}{$86.23\textcolor{gray}{\pm 0.03}$}  
&\multicolumn{1}{c}{$81.41\textcolor{gray}{\pm 0.12}$}  
%cmd
&\multicolumn{1}{c}{$83.68\textcolor{gray}{\pm 0.03}$}  
&\multicolumn{1}{c}{$82.59\textcolor{gray}{\pm 0.60}$}  
&\multicolumn{1}{c}{$78.03\textcolor{gray}{\pm 0.73}$}\\
\midrule
\multicolumn{16}{c}{Gradient Attack}\\%\midrule
\multicolumn{16}{c}{}  \\
Additive    
% sgd
&\multicolumn{1}{c}{-}  
&\multicolumn{1}{c}{-}  
&\multicolumn{1}{c}{-}  
% bgmd
&\multicolumn{1}{c}{$87.62\textcolor{gray}{\pm 0.10}$}  &\multicolumn{1}{c}{$87.87\textcolor{gray}{\pm 0.33}$}  &\multicolumn{1}{c}{$88.29\textcolor{gray}{\pm 0.01}$} 
% gmd
&\multicolumn{1}{c}{$88.38\textcolor{gray}{\pm 0.09}$}  &\multicolumn{1}{c}{$87.24\textcolor{gray}{\pm 0.16}$}  &\multicolumn{1}{c}{$83.89\textcolor{gray}{\pm 0.08}$}  
% cmd
&\multicolumn{1}{c}{$79.18\textcolor{gray}{\pm 0.26}$}  
&\multicolumn{1}{c}{$72.55\textcolor{gray}{\pm 0.16}$} 
&\multicolumn{1}{c}{$41.04\textcolor{gray}{\pm 1.13}$}\\ 
Bit Flip  
% sgd
&\multicolumn{1}{c}{$86.45\textcolor{gray}{\pm 0.11}$}  
&\multicolumn{1}{c}{-}  
&\multicolumn{1}{c}{-}  
% bgmd
&\multicolumn{1}{c}{$88.84\textcolor{gray}{\pm 0.20}$}  &\multicolumn{1}{c}{$88.42\textcolor{gray}{\pm 0.16}$}  &\multicolumn{1}{c}{$85.67\textcolor{gray}{\pm 0.09}$} 
% gmd
&\multicolumn{1}{c}{$88.61\textcolor{gray}{\pm 0.14}$}  &\multicolumn{1}{c}{$88.07\textcolor{gray}{\pm 0.05}$} &\multicolumn{1}{c}{$85.57\textcolor{gray}{\pm 0.14}$} 
% cmd
&\multicolumn{1}{c}{$83.91\textcolor{gray}{\pm 0.03}$}  
&\multicolumn{1}{c}{$84.20\textcolor{gray}{\pm 0.02}$}  
&\multicolumn{1}{c}{$82.33\textcolor{gray}{\pm 1.60}$}\\\midrule
\multicolumn{16}{c}{Label Attack}\\%\midrule
\multicolumn{16}{c}{}  \\
Backdoor  
% sgd
& \multicolumn{1}{c}{$88.42\textcolor{gray}{\pm 0.27}$}
& \multicolumn{1}{c}{$86.99\textcolor{gray}{\pm 0.02}$} 
& \multicolumn{1}{c}{$73.01\textcolor{gray}{\pm 0.68}$}
% bgmd
& \multicolumn{1}{c}{$89.19\textcolor{gray}{\pm 0.12}$} 
& \multicolumn{1}{c}{$88.97\textcolor{gray}{\pm 0.10}$} 
& \multicolumn{1}{c}{$84.69\textcolor{gray}{\pm 0.31}$}
% gmd
& \multicolumn{1}{c}{$88.84\textcolor{gray}{\pm 0.14}$}  
& \multicolumn{1}{c}{$88.26\textcolor{gray}{\pm 0.04}$} 
& \multicolumn{1}{c}{$81.32\textcolor{gray}{\pm 0.16}$}
% cmd
& \multicolumn{1}{c}{$80.91\textcolor{gray}{\pm 0.08}$}  
& \multicolumn{1}{c}{$76.38\textcolor{gray}{\pm 0.13}$} 
& \multicolumn{1}{c}{$60.85\textcolor{gray}{\pm 1.24}$}
\\\bottomrule
\end{tabular}}
\vspace{1 mm}
\caption{}
\label{table:fmnist_table}
\end{table}

==> result_table_main.tex <==
%%% FMNIST %%%%
\begin{table}[t]
\centering
\caption{\textbf{Homogeneous Training:} 1.12M parameter CNN trained on Fashion MNIST in regular i.i.d. setting. For all corruption types, test accuracy of \textsc{BGmD} is similar to that of \textsc{GmD} and surprisingly, in some cases even higher. As expected, \textsc{SGD} often diverges under corruption (empty entries in the table). \textsc{CmD} performs sub-optimally as corruption is increased.}
\vspace{1mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lllllllll@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{SGD} & \multicolumn{2}{c}{BGMD} & \multicolumn{2}{c}{GMD} & \multicolumn{2}{c}{CMD}\\%\cmidrule(lr){1-1}
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\textbf{Clean}    
& \multicolumn{2}{c}{$89.39\textcolor{gray}{\pm 0.28}$}   
& \multicolumn{2}{c}{$89.25 \textcolor{gray}{\pm 0.19}$}     
& \multicolumn{2}{c}{$88.98\textcolor{gray}{\pm 0.3}$}    
& \multicolumn{2}{c}{$83.82\textcolor{gray}{\pm 0.26}$} \\ %\midrule
\multicolumn{9}{c}{}  \\
Corruption (\%)             &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}       &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}        &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}      &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}\\\midrule

\multicolumn{9}{c}{Feature Attack}                         \\%\midrule
\multicolumn{9}{c}{}  \\
Additive 
%sgd
& \multicolumn{1}{c}{-} 
& \multicolumn{1}{c}{-}
%bgmd
& \multicolumn{1}{c}{$86.76\textcolor{gray}{\pm 0.03}$} 
& \multicolumn{1}{c}{$82.27\textcolor{gray}{\pm 0.06}$}
%gmd
& \multicolumn{1}{c}{$86.63\textcolor{gray}{\pm 0.04}$} 
& \multicolumn{1}{c}{$81.23\textcolor{gray}{\pm 0.03}$} 
%cmd
& \multicolumn{1}{c}{$82.38\textcolor{gray}{\pm 0.13}$} 
& \multicolumn{1}{c}{$78.54\textcolor{gray}{\pm 0.65}$}
\\
Impulse    
%sgd
&\multicolumn{1}{c}{$79.18\textcolor{gray}{\pm 6.47}$}  
&\multicolumn{1}{c}{-} 
%bgmd 
&\multicolumn{1}{c}{$86.91\textcolor{gray}{\pm 0.36}$}  
&\multicolumn{1}{c}{$81.73\textcolor{gray}{\pm 0.06}$} 
%gmd
&\multicolumn{1}{c}{$86.23\textcolor{gray}{\pm 0.03}$}  
&\multicolumn{1}{c}{$81.41\textcolor{gray}{\pm 0.12}$}  
%cmd
&\multicolumn{1}{c}{$82.59\textcolor{gray}{\pm 0.60}$}  
&\multicolumn{1}{c}{$78.03\textcolor{gray}{\pm 0.73}$}\\
\midrule
\multicolumn{9}{c}{Gradient Attack}\\%\midrule
\multicolumn{9}{c}{}  \\
Additive    
% sgd
&\multicolumn{1}{c}{-}  
&\multicolumn{1}{c}{-}  
% bgmd
  &\multicolumn{1}{c}{$87.87\textcolor{gray}{\pm 0.33}$}  &\multicolumn{1}{c}{$88.29\textcolor{gray}{\pm 0.01}$} 
% gmd
 &\multicolumn{1}{c}{$87.24\textcolor{gray}{\pm 0.16}$}  &\multicolumn{1}{c}{$83.89\textcolor{gray}{\pm 0.08}$}  
% cmd  
&\multicolumn{1}{c}{$72.55\textcolor{gray}{\pm 0.16}$} 
&\multicolumn{1}{c}{$41.04\textcolor{gray}{\pm 1.13}$}\\ 
Bit Flip  
% sgd
&\multicolumn{1}{c}{-}  
&\multicolumn{1}{c}{-}  
% bgmd
&\multicolumn{1}{c}{$88.42\textcolor{gray}{\pm 0.16}$}  &\multicolumn{1}{c}{$85.67\textcolor{gray}{\pm 0.09}$} 
% gmd
&\multicolumn{1}{c}{$88.07\textcolor{gray}{\pm 0.05}$} &\multicolumn{1}{c}{$85.57\textcolor{gray}{\pm 0.14}$} 
% cmd
&\multicolumn{1}{c}{$84.20\textcolor{gray}{\pm 0.02}$}  
&\multicolumn{1}{c}{$82.33\textcolor{gray}{\pm 1.60}$}\\\midrule
\multicolumn{9}{c}{Label Attack}\\%\midrule
\multicolumn{9}{c}{}  \\
Backdoor  
% sgd
& \multicolumn{1}{c}{$86.99\textcolor{gray}{\pm 0.02}$} 
& \multicolumn{1}{c}{$73.01\textcolor{gray}{\pm 0.68}$}
% bgmd
& \multicolumn{1}{c}{$88.97\textcolor{gray}{\pm 0.10}$} 
& \multicolumn{1}{c}{$84.69\textcolor{gray}{\pm 0.31}$}
% gmd
& \multicolumn{1}{c}{$88.26\textcolor{gray}{\pm 0.04}$} 
& \multicolumn{1}{c}{$81.32\textcolor{gray}{\pm 0.16}$}
% cm
& \multicolumn{1}{c}{$76.38\textcolor{gray}{\pm 0.13}$} 
& \multicolumn{1}{c}{$60.85\textcolor{gray}{\pm 1.24}$}\\\bottomrule
\end{tabular}}
\vspace{0mm}
\label{table:fmnist_table}
\end{table}


%% CIFAR %%
\begin{table}[t]
\centering
\caption{\textbf{Heterogeneous Training:} ResNet-18 trained on CIFAR-10 in a federated setting. \textsc{GmD} and \textsc{BGmD} both remain robust at both 20\% and 40\% corruption maintaining high accuracy. Interestingly, even in non-corrupt setting, \textsc{BGmD} outperforms \textsc{SGD}, perhaps due to the distributional shift introduced by non-i.i.d setting. Recall that in i.i.d setting, our model achieves 94.8\% accuracy with \textsc{SGD}}
\vspace{1mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lllllllll@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{SGD} & \multicolumn{2}{c}{BGMD} & \multicolumn{2}{c}{GMD} & \multicolumn{2}{c}{CMD}\\%\cmidrule(lr){1-1}
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\textbf{Clean}    
& \multicolumn{2}{c}{$82.29^*\textcolor{gray}{\pm 1.32}$}   
& \multicolumn{2}{c}{$84.82 \textcolor{gray}{\pm 0.76}$}     
& \multicolumn{2}{c}{$85.65\textcolor{gray}{\pm 0.48}$}    
& \multicolumn{2}{c}{$85.50\textcolor{gray}{\pm 1.43}$} \\ %\midrule
\multicolumn{9}{c}{}  \\
Corruption (\%)             &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}       &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}        &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}      &\multicolumn{1}{c}{20}    &\multicolumn{1}{c}{40}\\\midrule
Bit Flip  
% sgd
&\multicolumn{1}{c}{-}  
&\multicolumn{1}{c}{-}  
% bgmd
  &\multicolumn{1}{c}{$84.56\textcolor{gray}{\pm 0.06}$} 
  &\multicolumn{1}{c}{$82.66\textcolor{gray}{\pm 0.31}$}
% gmd
&\multicolumn{1}{c}{$88.07\textcolor{gray}{\pm 0.05}$} &\multicolumn{1}{c}{$80.87\textcolor{gray}{\pm 0.01}$} 
% cmd
&\multicolumn{1}{c}{$80.87\textcolor{gray}{\pm 0.21}$}  
&\multicolumn{1}{c}{$77.41\textcolor{gray}{\pm 1.04}$}\\\bottomrule
\end{tabular}}
\vspace{-4mm}
\label{table:cifar_table}
\end{table}

==> supp_exp.tex <==
\section{Effectiveness and Limitations of \textsc{BGmD}}
Intuitively, as a consequence of over-parameterization, large scale deep learning models are likely to have sparse gradient estimates \cite{shi2019understanding}. In the context of robust optimization this would imply that performing robust gradient estimation in a low-dimensional subspace has little to no impact in the downstream optimization task especially in case of over-parameterized models.
Thus, by judiciously selecting a block of co-ordinates and performing robust gradient estimation only in this low-dimensional subspace is a practical approach to leverage highly robust estimators such as \textsc{Gm} even in high dimensional setting which was previously intractable. This means \textsc{BGmD} would be an attractive choice especially in overparameterized setting. In order to validate this, we perform a small experiment: we take a tiny 412 parameter CNN and a large 1.16M parameter CNN and train both on simple MNIST dataset. In addition to looking at the train and test performance we also compute relative residual error $1 - \xi = \|\mG_t - \gC_k(\mG_t)\|_F^2/\|\mG_t\|_F^2$  Lemma~\ref{lemma:norm_sampling} at each gradient step (iteration). We plot the relative residual, train and test performance for different values of $k = \beta d$ where $0 < \beta \leq 1$ in Figure~\ref{figure:supp.role.k.lenet}, ~\ref{figure:supp.role.k.tiny}. \footnote{Just to clarify, both these experiments are performed in clean setting}

\begin{figure}[htb]
\subfloat[\footnotesize{Relative Residual}]{\includegraphics[width=0.33\columnwidth]{figs/neurips/supp/role_k_lenet_residual.png}}
\subfloat[\footnotesize{Test Accuracy}]{\includegraphics[width=0.33\columnwidth]{figs/neurips/supp/role_k_lenet_test.png}}
\subfloat[\footnotesize{Train Loss}]{\includegraphics[width=0.33\columnwidth]{figs/neurips/supp/role_k_lenet_train.png}}
\caption{\footnotesize{\textbf{Large Model}: We train an over-parameterized ($d$ = 1.16 M) parameter CNN on MNIST~\cite{lecun1998gradient} dataset. (a) shows relative residual error as a function of iterations (gradient steps) (b) and (c) show the corresponding test and training performance. The residual error starts to approaches zero as training progresses even for very small values of $k$ explaining negligible impact on training and test performance.}} 
\label{figure:supp.role.k.lenet}
\end{figure}

\begin{figure}[htb]
\subfloat[\footnotesize{Relative Residual}]{\includegraphics[width=0.33\columnwidth]{figs/neurips/supp/role_k_tiny_residual.png}}
\subfloat[\footnotesize{Test Accuracy}]{\includegraphics[width=0.33\columnwidth]{figs/neurips/supp/role_k_tiny_test.png}}
\subfloat[\footnotesize{Train Loss}]{\includegraphics[width=0.33\columnwidth]{figs/neurips/supp/role_k_tiny_train.png}}
\caption{\footnotesize{\textbf{Tiny Model}: Here we instead train a super tiny $d=412$ parameter CNN on MNIST. (a),(b),(c) plots relative residual, train and test performance respectively. We can see that even in this setting $(1 - \xi) > k/d = \beta$ as we remarked in Lemma~\ref{lemma:norm_sampling}. However, as training progresses the gradients become closer to uniform explaining the optimality gap of \textsc{BGmD} with small values of $k$.}}
\label{figure:supp.role.k.tiny}
\end{figure}
\vspace{1mm}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
It is clear from these experiments that in over-parameterized settings $1 \xi \to 0$ as training progresses potentially due to the inherent sparsity of overparameterized models. This implies our block selection procedure is often near lossless and thus \textsc{BGmD} even with aggressively small $k$ can achieve near optimal performance. And since it is a few orders of magnitude faster than \textsc{GmD} - it is an attractive robust optimization algorithm in high dimensions. However, in the tiny CNN setting, as training progresses the gradients tend to become more uniform ~ implying higher loss due to block co-ordinate selection. This implies, in these settings, \textsc{BGmD} needs to use a larger $k$ in order to retain the optimal performance. However, note that in these small scale settings, \textsc{GmD} is not expensive and thus for robust optimization , a larger value of $k$ or at the extreme $k=d$ i.e. running \textsc{GmD} can be practical. 

\section{Additional Robustness Experiments}

\begin{table}[htb!]
\centering
\caption{1.12M parameter CNN trained on MNIST in regular i.i.d. setting. For all corruption types, test accuracy of \textsc{BGmD} is similar to that of \textsc{GmD} and surprisingly, in some cases even higher. As expected, \textsc{SGD} fails to make progress under corruption . \textsc{CmD} performs sub-optimally as corruption is increased.}
\begin{tabular}{llllll}
\toprule
& Corruption (\%) 
& \multicolumn{1}{c}{SGD} 
& \multicolumn{1}{c}{\textsc{CmD}} 
& \multicolumn{1}{c}{\textsc{BGmD}} 
& \multicolumn{1}{c}{\textsc{GmD}} \\ \midrule
Clean             
& \multicolumn{1}{c}{-}   
& \multicolumn{1}{c}{$\mathbf{99.27}\textcolor{gray}{\pm 0.01}$}    
& \multicolumn{1}{c}{$98.83\textcolor{gray}{\pm 0.02}$}    
& \multicolumn{1}{c}{$99.09\textcolor{gray}{\pm 0.05}$}     
& \multicolumn{1}{c}{$99.24\textcolor{gray}{\pm 0.02}$}    \\
\multicolumn{6}{c}{}\\
\multicolumn{6}{c}{Gradient Attack}\\
\multicolumn{6}{c}{}\\
\multirow{2}{*}{Bit Flip} 
& \multicolumn{1}{c}{20}
& \multicolumn{1}{c}{$9.51\textcolor{gray}{\pm 1.77}$}    
& \multicolumn{1}{c}{$98.79\textcolor{gray}{\pm 0.01}$}    
& \multicolumn{1}{c}{$\mathbf{99.06}\textcolor{gray}{\pm 0.02}$}     
& \multicolumn{1}{c}{$98.98\textcolor{gray}{\pm 0.01}$}    \\
& \multicolumn{1}{c}{40}             
& \multicolumn{1}{c}{$9.60\textcolor{gray}{\pm 2.04}$}     
& \multicolumn{1}{c}{$93.69\textcolor{gray}{\pm 0.09}$}     
& \multicolumn{1}{c}{$97.89\textcolor{gray}{\pm 0.05}$}      
& \multicolumn{1}{c}{$\mathbf{98.11}\textcolor{gray}{\pm 0.12}$} \\
\multicolumn{6}{c}{}\\
\multirow{2}{*}{Additive} 
& \multicolumn{1}{c}{20}
& \multicolumn{1}{c}{$9.68\textcolor{gray}{\pm 0.11}$}     
& \multicolumn{1}{c}{$94.26\textcolor{gray}{\pm 0.03}$}     
& \multicolumn{1}{c}{$98.61\textcolor{gray}{\pm 0.01}$}      
& \multicolumn{1}{c}{$\mathbf{98.69}\textcolor{gray}{\pm 0.01}$}    \\
& \multicolumn{1}{c}{40}             
& \multicolumn{1}{c}{$9.74\textcolor{gray}{\pm 0.12}$}     
& \multicolumn{1}{c}{$91.86\textcolor{gray}{\pm 0.03}$}    
& \multicolumn{1}{c}{$\mathbf{97.78}\textcolor{gray}{\pm 0.27}$}      
& \multicolumn{1}{c}{$92.78\textcolor{gray}{\pm 0.04}$} \\\bottomrule 
\end{tabular}
\label{table:supp.mnist}
\end{table}
\vspace{5mm}

\begin{table}[htb!]
\centering
\caption{This is an extension of Table~\ref{table:cifar_table} we present results on two different gradient attack models. We see similar trends at high corruptions \textsc{GmD} achieves similar or even better performance than \textsc{BGmD} while taking ~3x less time}
\begin{tabular}{llllll}
\toprule
& Corruption (\%) 
& \multicolumn{1}{c}{SGD} 
& \multicolumn{1}{c}{\textsc{CmD}} 
& \multicolumn{1}{c}{\textsc{BGmD}} 
& \multicolumn{1}{c}{\textsc{GmD}} \\ \midrule
Clean             
& \multicolumn{1}{c}{-}   
& \multicolumn{1}{c}{$82.29\textcolor{gray}{\pm 1.32}$}    
& \multicolumn{1}{c}{$85.50\textcolor{gray}{\pm 1.43}$}    
& \multicolumn{1}{c}{$84.82\textcolor{gray}{\pm 0.76}$}     
& \multicolumn{1}{c}{$\mathbf{85.65}\textcolor{gray}{\pm 0.48}$}    \\
\multicolumn{6}{c}{}\\
\multicolumn{6}{c}{Gradient Attack}\\
\multicolumn{6}{c}{}\\
\multirow{2}{*}{Bit Flip} 
& \multicolumn{1}{c}{20}
& \multicolumn{1}{c}{-}    
& \multicolumn{1}{c}{$80.87\textcolor{gray}{\pm 0.21}$}    
& \multicolumn{1}{c}{${84.56}\textcolor{gray}{\pm 0.06}$}     
& \multicolumn{1}{c}{$\mathbf{88.07}\textcolor{gray}{\pm 0.05}$}    \\
& \multicolumn{1}{c}{40}             
& \multicolumn{1}{c}{-}     
& \multicolumn{1}{c}{$77.41\textcolor{gray}{\pm 1.04}$}     
& \multicolumn{1}{c}{$\mathbf{82.66}\textcolor{gray}{\pm 0.31}$}      
& \multicolumn{1}{c}{$80.81\textcolor{gray}{\pm 0.01}$} \\
\multicolumn{6}{c}{}\\
\multirow{2}{*}{Additive} 
& \multicolumn{1}{c}{20}
& \multicolumn{1}{c}{$20.7\textcolor{gray}{\pm 1.56}$}     
& \multicolumn{1}{c}{$54.75\textcolor{gray}{\pm 0.38}$}     
& \multicolumn{1}{c}{$\mathbf{83.84}\textcolor{gray}{\pm 0.12}$}      
& \multicolumn{1}{c}{$82.40\textcolor{gray}{\pm 0.90}$}    \\
& \multicolumn{1}{c}{40}             
& \multicolumn{1}{c}{-}     
& \multicolumn{1}{c}{$23.35\textcolor{gray}{\pm 6.13}$}    
& \multicolumn{1}{c}{$\mathbf{82.79}\textcolor{gray}{\pm 0.68}$}      
& \multicolumn{1}{c}{$79.46\textcolor{gray}{\pm 0.24}$} \\\bottomrule 
\end{tabular}
\label{table:supp.cifar}
\end{table}

\begin{figure}[htb!]
\subfloat[\footnotesize{No corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/fmnist/clean.png}}
\subfloat[\footnotesize{10\% Corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/supp/fmnist.backdoor10.png}}
\subfloat[\footnotesize{20\% Corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/supp/fmnist.backdoor20.png}}
\subfloat[\footnotesize{40\% Corruption}]{\includegraphics[width=0.25\columnwidth]{figs/neurips/supp/fmnist.backdoor40.png}}  
\caption{\footnotesize{\textbf{Robustness to Label Corruption}: We train a CNN on Fashion-MNIST in the i.i.d setting in presence of \textbf{backdoor attack}. \textsc{BGmD} achieves up to large speedup over \textsc{GmD} while being robust even at very high corruptions where \textsc{SGD} converges very slowly due to backdoor attack and converges to a sub-optimal point at high 40\% corruption.\textsc{CmD} converges to sub-optimal solution.}}
\label{figure:fmnist.label_corr}
% \vspace{-5mm} 
\end{figure}

==> theory_fed_bgmd.tex <==
Similar to the proof of \textsc{BGmD}, we first, we define the average of non-corrupt local functions:
\begin{equation}
\label{equation:true_f.fl}
    f(\vx):= \frac{1}{|\sG|}\sum_{i\in \sG} f_i(\vx).
\end{equation}
We further assume that Assumption \ref{assumption:period} holds in this setting. Now we can establish the following results similar to \textsc{BgmD} under smooth non-convex and non-convex satisfying PLC settings. The complete statements and proof can be found in the Appendix. 

\begin{theorem}[\bf Non-convex]
\label{theorem:non_convex_simple.fl}
Consider the general case where the functions $f_i$ corresponding to non-corrupt samples $i \in \sG$ in \eqref{equation:true_f.fl} are \textbf{non-convex} and \textbf{smooth} (Assumption \ref{assumption:smooth}). Define, $R_0 := f(\vx_0)-f(\vx^\ast)$ where $\vx^\ast$ is the true optima and $\vx_0$ is the initial parameters. Run Algorithm \ref{algorithm:full.fl} with compression factor $(1 - \beta_{k,s})\frac{k}{d} \leq \xi \leq 1$ (Lemma \ref{lemma:qsparse}), learning rate $\gamma =  1/2L$ and $\epsilon-$approximate \textup{\textsc{Gm}($\cdot$)} oracle in presence of $\alpha-$corruption (Definition \ref{definition:byzantine}) for $T$ iterations. Then the iterates satisfy:
\begin{equation}
\begin{aligned}
\frac{1}{T|\sG|} \sum_{t=0}^{T-1}\sum_{i\in\sG}\text{ }\E\|  \nabla f(\vy_t^i)\|^2 \leq &\frac{8R_0}{\gamma T}+8L\gamma\sigma^2+24 L^2 \gamma^2H^2\sigma^2\left[1+\frac{4(1-\xi^2)}{\xi^2}\right] \\
& + \frac{2304 |\gI_T|H^2\sigma^2}{T(1-\alpha)^2}\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]+\frac{48|\gI_T|\epsilon^2}{\gamma^2T|\sG|^2(1-\alpha)^2}\end{aligned}
\end{equation}
\end{theorem}

\begin{theorem}[\textbf{Non-convex under PLC}]
\label{theorem:plc_simple.fl}
Consider that functions $f_i$ in \eqref{equation:true_f.fl} are \textbf{non-convex} and also satisfies the \textbf{Polyak-\L{}ojasiewicz Condition} (Assumption \ref{assumption:plc}) with parameter $\mu$. Define, $R_0 := f(\vx_0)-f(\vx^\ast)$ where $\vx^\ast$ is the true optima and $\vx_0$ is the initial parameters. After $T$ iterations Algorithm \ref{algorithm:full.fl} with compression factor $(1 - \beta_{k,s})\frac{k}{d} \leq \xi \leq 1$ (Lemma \ref{lemma:qsparse}), learning rate $\gamma =  1/4L$ and $\epsilon-$approximate \textup{\textsc{Gm}($\cdot$)} oracle in presence of $\alpha-$corruption (Definition \ref{definition:byzantine}) satisfies:
\begin{equation}
\begin{aligned}
\frac{1}{|\sG|}\sum_{i\in\sG} \text{ }\E\|\hat{\vy}_T^i-\vx^\ast\|^2 \leq &\frac{16(f(\vx_0)-f^\ast)}{\mu^2\gamma}\left[1-\frac{\mu\gamma}{2}\right]^T + \frac{16L\gamma\sigma^2}{\mu^2} + \frac{40 L^2}{\mu^2} \gamma^2H^2\sigma^2\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]\\
&+\frac{3072 H^2\sigma^2}{\mu^2(1-\alpha)^2}\left[1+\frac{4(1-\xi^2)}{\xi^2}\right]+\frac{64\epsilon^2}{\mu^2\gamma^2 |\sG|^2(1-\alpha)^2},
 \end{aligned}
 \end{equation}
for a global optimal solution  $\vx^\ast \in \gX^\ast$. Here,
$\hat{\vy}_T^i := \frac{1}{W_T}\sum_{t=0}^{T-1}w_t\vy_t^i$ with weights given as $w_t := (1-\frac{\mu\gamma}{2})^{-(t+1)}$, $W_T := \sum_{t=0}^{T-1}w_t$.
%  where $w_t = (1-\frac{\mu\gamma}{2})^{-(t+1)}$, $W_T = \sum_{t=0}^{T-1}w_t$, and $\vq^i_t \in \gX^\ast$, for all $i\in \sG$ and $t=0,\dots T-1$.
\end{theorem}
